The Illusion of Readiness in Health AI

Large language models have demonstrated remarkable performance in a wide range of medical benchmarks. Yet underneath the seemingly promising results lie salient growth areas, especially in cutting-edge frontiers such as multimodal reasoning. In this paper, we introduce a series of adversarial stress tests to systematically assess the robustness of flagship models and medical benchmarks. Our study reveals prevalent brittleness in the presence of simple adversarial transformations: leading systems can guess the right answer even with key inputs removed, yet may get confused by the slightest prompt alterations, while fabricating convincing yet flawed reasoning traces. Using clinician-guided rubrics, we demonstrate that popular medical benchmarks vary widely in what they truly measure. Our study reveals significant competency gaps of frontier AI in attaining real-world readiness for health applications. If we want AI to earn trust in healthcare, we must demand more than leaderboard wins and must hold AI systems accountable to ensure robustness, sound reasoning, and alignment with real medical demands.

==> arxiv2510/sections_v0/benchmark.tex <==
% \section{Benchmark Comparisons}
% Preliminary evaluation highlights how visual chain-of-thought reasoning improves interpretability and accuracy in some tasks. In this section, we compare GPT-4o and GPT o3 on expert-scored MRI tumor localization.
\begin{table}[ht]
\centering
\caption{Benchmark accuracy across medical visual question answering and report tasks.}
\begin{tabularx}{\textwidth}{@{}l c c c X@{}}
\toprule
\textbf{Benchmark} & \textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule

\multirow{4}{*}{VQA-RAD} 
  & GPT-4o             & 100 & 50\% \\
  & GPT-o3             & 100 & 58\% \\
  & GPT-4o + CoT       & 100 & 47\% \\
  & GPT-o3 + CoT       & 100 & 54\% \\
  
\addlinespace
\multirow{12}{*}{PMC-VQA}
  & GPT-4o             & 100 & 47.00\% \\
  & GPT-4o             & 95 & 48.42\% \\
  & GPT-o3-zero        & 95 & 55.79\%/60.00\% \\
  & GPT-o3-low         & 95 & 52.63\% \\
  & GPT-o3-medium      & 95 & 57.89\% \\
  & GPT-o3-high        & 95 & 57.89\% \\
  & GPT-o4-mini-zero   & 95 & 57.89\% \\
  & GPT-o4-mini-low    & 95 & 57.89\% \\
  & GPT-o4-mini-medium & 95 & 52.63\% \\
  & GPT-o4-mini-high   & 95 & 55.21\% \\
  & Gemini-2.5-pro     & 100& 62.00\% \\
  & Gemini-2.5-pro     & 95 & 62.11\% \\
  & GPT-4o             & 500 & 49.80\% \\
  & GPT-4o             & 486 & 50.21\% \\
  & GPT-o3-zero        & 486 & 60.08\% \\
  & GPT-o4-mini-zero   & 486 & 59.47\% \\
  & Gemini-2.5-pro     & 500 & 58.80\%\\
  & Gemini-2.5-pro     & 486 & 58.44\%\\
  
\addlinespace
\multirow{11}{*}{OmniMedVQA}
  & GPT-4o             & 105 & 74.29\% \\
  & GPT-o3-zero        & 105 & 87.62\% \\
  & GPT-o3-low         & 105 & 88.57\% \\
  & GPT-o3-medium      & 105 & 87.62\% \\
  & GPT-o3-high        & 105 & 88.57\% \\
  & GPT-o4-mini-zero   & 105 & 83.81\% \\
  & GPT-o4-mini-low    & 105 & 83.81\% \\
  & GPT-o4-mini-medium & 105 & 85.71\% \\
  & GPT-o4-mini-high   & 105 & 86.67\% \\
  & Gemini-2.5-flash   & 105 & 79.05\% \\
  & Gemini-2.5-pro     & 105 & 87.62\% \\
  & LLava-Med          & 105 & 68.57\% \\
  & GPT-4o             & 524 & 73.09\% \\
  & GPT-o3-zero        & 517 & 84.91/85.49\% \\  
  & GPT-o4-mini-zero   & 517 & 81.43\% \\
  & Gemini-2.5-pro     & 524 & 85.69\% \\
  & Gemini-2.5-pro     & 517 & 85.69\% \\
  & LLava-Med          & 524 & 68.70\% \\

  
% \addlinespace
% \multirow{2}{*}{MIMIC-CXR}
%   & GPT-4o             & 100 & 36\% \\
%   & GPT-o3             & 100 & 36\% \\
  
\addlinespace
\multirow{2}{*}{JAMA}
  & GPT-4o             & 1314 & 73.97\% \\
  & GPT-4o             & 1086 (content filter) & 73.94\% \\
  & GPT-o3-zero        & 1086 (content filter) & 86.56\% \\ 
  & GPT-o4-mini-zero   & 1086 (content filter) & 85.91\% \\
  & Gemini-2.5-pro     & 1314 & 69.33\% \\
  & Gemini-2.5-pro     & 1086 (content filter) & 67.68\%\\
  & GPT-4o (text)      & 1314 &  68.34\% \\
  & GPT-o3 (text)      & 1314 &  82.42\% \\
  & GPT-o4-mini (text) & 1314 &  77.70\% \\
  & Gemini-2.5-pro (text)     & 1314 &  74.58\% \\
  & LLava-Med          & 1314 & 21.40\% \\

\addlinespace
\multirow{2}{*}{NEJM}
  & GPT-4o             & 947 & 66.53\% \\
  & GPT-4o             & 743 & 66.90\% \\
  & GPT-o3  zero       & 743 (content filter) & 80.89\% \\ 
  & GPT-o4-mini zero   & 743 (content filter) & 75.91\% \\
  & Gemini-2.5-pro     & 947 & 80.89\%\\
  & Gemini-2.5-pro     & 743 & 79.95\%\\
  & GPT-4o (text)      & 947 & 37.38\% \\
  & GPT-o3 (text)      & 947 & 67.69\% \\ 
  & GPT-o4-mini(text)  & 947 & 66.42\% \\
  & Gemini-2.5-pro(text)    & 947 & 74.58\% \\
  
\bottomrule
\end{tabularx}
\end{table}


% \section{Benchmark Comparisons}
% Preliminary evaluation highlights how visual chain-of-thought reasoning improves interpretability and accuracy in some tasks. In this section, we compare GPT-4o and GPT o3 on expert-scored MRI tumor localization.
% \begin{table}[ht]
% \centering
% \caption{Benchmark accuracy across medical visual question answering and report tasks.}
% \begin{tabularx}{\textwidth}{@{}l c c c X@{}}
% \toprule
% \textbf{Benchmark} & \textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
% \midrule
  
% \addlinespace
% \multirow{4}{*}{OmniMedVQA}
%   & GPT-4o             & 524 & 73.11 (0.2532)\% \\
%   & GPT-o3-low        & 517 & 84.91 (0.2235)\% \\  
%   & GPT-o3-medium    & 517 & 84.99 (0.1274)\% \\
%   & GPT-o3-high      & 524 & 85.84 (0.3492)\% \\

% % GPT-4o              73.09%, 72.92%, 72.73%, 72.73%, 74.08% 
% % GPT-o3-low          85.49%, 84.72%, 84.14%, 84.91%, 85.30%
% % GPT-o3-medium       85.49%, 84.53%, 84.91%, 85.30%, 84.72%
% % GPT-o3-high         86.46%, 85.30%, 85.49%, 86.65%， 85.30%

% \bottomrule
% \end{tabularx}
% \end{table}


\begin{table}[ht]
\centering
\caption{Performance on the VQA-RAD benchmark, a short-form single-modality visual question answering dataset focused on radiographic reasoning.}
\label{tab:vqa_rad}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o         & 100 & 50\% \\
GPT-o3         & 100 & 58\% \\
GPT-4o + CoT   & 100 & 47\% \\
GPT-o3 + CoT   & 100 & 54\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Results on PMC-VQA, a cross-modality benchmark containing open-ended questions grounded in biomedical literature and image context.}
\label{tab:pmc_vqa}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o             & 486 & 50.21\% \\
GPT-o3-zero        & 486 & 60.08\% \\
GPT-o3-low         & 486 & 52.63\% \\
GPT-o3-medium      & 486 & 57.89\% \\
GPT-o3-high        & 486 & 57.89\% \\
GPT-o4-mini-zero   & 486 & 57.89\% \\
Gemini-2.5-pro     & 486 & 58.44\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Performance on OmniMedVQA, a comprehensive benchmark spanning 73 medical datasets and 12 imaging modalities, designed to evaluate generalist medical visual reasoning.}
\label{tab:omnimedvqa}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o             & 524 & 73.11\% \\
GPT-o3-low         & 524 & 84.91\% \\
GPT-o3-medium      & 524 & 84.99\% \\
GPT-o3-high        & 524 & 85.84\% \\
GPT-o4-mini-zero   & 524 & 81.43\% \\
Gemini-2.5-pro     & 524 & 85.69\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Accuracy on challenging real-world case questions from JAMA Clinical Challenge and NEJM Case Reports. These benchmarks assess multi-step reasoning and domain-specific clinical understanding.}
\label{tab:clinical_cases}
\begin{tabular}{lcc}
\toprule
\textbf{Benchmark} & \textbf{Model} & \textbf{Accuracy} \\
\midrule
JAMA   & GPT-o3-zero      & 86.56\% \\
JAMA   & Gemini-2.5-pro   & 69.33\% \\
NEJM   & GPT-o3-zero      & 80.89\% \\
NEJM   & Gemini-2.5-pro   & 80.89\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Model accuracy on JAMA clinical case challenge.}  
JAMA cases are predominantly solvable via text alone.  
Text-only models perform competitively, and in some cases (e.g., Gemini-2.5-pro), outperform their multimodal counterparts.   
Filtered inputs reflect examples where image access was blocked by safety mechanisms.}

\begin{tabular}{llcc}
\toprule
\textbf{Model} & \textbf{Input Type} & \textbf{\# Examples} & \textbf{Accuracy (\%)} \\
\midrule
GPT-o3        & Image + Text (filtered) & 1086 & \textbf{86.56} \\
GPT-o4-mini   & Image + Text (filtered) & 1086 & 85.91 \\
GPT-4o             & Image + Text            & 1314 & 73.97 \\
GPT-4o             & Image + Text (filtered) & 1086 & 73.94 \\
Gemini-2.5-pro     & Image + Text            & 1314 & 69.33 \\
Gemini-2.5-pro     & Image + Text (filtered) & 1086 & 67.68 \\
LLaVA-Med          & Image + Text            & 1314 & 21.40 \\
\addlinespace
GPT-o3             & Text Only               & 1314 & \textbf{82.42} \\
GPT-o4-mini        & Text Only               & 1314 & 77.70 \\
Gemini-2.5-pro     & Text Only               & 1314 & 74.58 \\
GPT-4o             & Text Only               & 1314 & 68.34 \\
\bottomrule
\end{tabular}
\label{tab:jama_cases}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Model accuracy on NEJM clinical case challenge.} These tasks require visual reasoning and context integration. Multimodal models clearly outperform text-only models.}
\begin{tabular}{llcc}
\toprule
\textbf{Model} & \textbf{Input Type} & \textbf{\# Examples} & \textbf{Accuracy (\%)} \\
\midrule
Gemini-2.5-pro     & Image + Text           & 947 & \textbf{80.89} \\
GPT-o3-zero        & Image + Text (filtered) & 743 & \textbf{80.89} \\
Gemini-2.5-pro     & Image + Text (filtered) & 743 & 79.95 \\
GPT-o4-mini-zero   & Image + Text (filtered) & 743 & 75.91 \\
GPT-4o             & Image + Text           & 947 & 66.53 \\
GPT-4o             & Image + Text (filtered) & 743 & 66.90 \\
\addlinespace
Gemini-2.5-pro     & Text Only              & 947 & \textbf{74.58} \\
GPT-o3             & Text Only              & 947 & 67.69 \\
GPT-o4-mini        & Text Only              & 947 & 66.42 \\
GPT-4o             & Text Only              & 947 & 37.38 \\
\bottomrule
\end{tabular}
\label{tab:nejm_cases}
\end{table}


\section{Failure to Reason: Empirical Analysis of State‑of‑the‑Art VLMs}
\label{sec:failure_to_reason}

Despite strong benchmark performance, current vision–language models (VLMs) exhibit critical limitations when evaluated on clinically grounded reasoning tasks. We assess five frontier models—GPT–4o, GPT–o3, GPT–o4‑mini, Gemini‑2.5\,pro, and LLaVA‑Med—across four carefully chosen task categories that span the spectrum of visual and textual complexity in real‑world clinical workflows.

\paragraph{Task Selection Rationale.}
To capture the diversity of multimodal clinical reasoning, we structure our evaluation along four axes: (1)~image-only VQA for visual pattern recognition, (2)~cross‑modal VQA for basic alignment of image and text cues, (3)~real-world diagnostic challenges that reflect authentic physician workflows, and (4)~free‑form report generation for end-to-end summarization. This progression reflects increasing demands in contextualization, temporal reasoning, and interpretability—capabilities essential for deployment in healthcare.

\subsection{Performance Across Clinical Tasks}

\textbf{Image‑only VQA (VQA‑RAD).}
Performance is modest across models (50–58\,\%); chain‑of‑thought (CoT) prompting introduces verbosity without consistent gains, suggesting shallow template reasoning (Table~\ref{tab:vqa_rad}).

\textbf{Cross‑modal VQA (PMC‑VQA; OmniMedVQA).}
Gemini‑2.5‑pro and GPT–o3‑high exceed 85 \% accuracy (Tables~\ref{tab:pmc_vqa},\ref{tab:omnimedvqa}), though qualitative review reveals brittleness to phrasing variation and domain shifts.

\textbf{Clinical case reasoning (JAMA vs.\ NEJM).}
JAMA tasks are largely text-resolvable: GPT–o3 (text-only) attains 82.4 \%, exceeding many multimodal configurations. Yet when visual grounding is required—as in NEJM—multimodal models like GPT–o3-zero and Gemini‑2.5‑pro outperform text-only inputs by 6–9 pp, reaching up to 80.9 \% (Tables~\ref{tab:jama_cases},\ref{tab:nejm_cases}).

\textbf{Report generation (MIMIC‑CXR).}
Models hallucinate confident but unsupported impressions, omit clinically subtle findings, and inconsistently integrate prior context. Standard lexical metrics fail to penalize these issues meaningfully.

\subsection{Common Failure Patterns}

\begin{enumerate}[label=(\roman*)]
    \item \textbf{Hallucinated findings.} Confident but spurious pathologies are generated in $\sim$18\,\% of MIMIC-CXR samples (human audit, $n{=}200$).
    \item \textbf{Spatial confusion.} Laterality and anatomical misattribution are common in brain and chest tasks.
    \item \textbf{Temporal neglect.} When presented with prior studies, models fail to detect interval change or disease progression.
    \item \textbf{Template reasoning.} CoT outputs often recycle generic logic without case-specific visual grounding.
\end{enumerate}

\subsection{Modality-Dependent Insights from JAMA and NEJM}

Table~\ref{tab:benchmark_comparison} summarizes modality effects. In JAMA, where textual cues dominate, LLMs achieve strong performance with or without images. In NEJM, multimodal inputs substantially improve accuracy, revealing that current models struggle when image-grounded reasoning is essential. This contrast highlights the importance of benchmark design in surfacing meaningful deficits.

\subsection{Emergent Visual Reasoning via Image Manipulation}
\label{sec:visual_case_studies}

Although current APIs for models like GPT–4o and GPT–o3 do not yet support reasoning over images via fine-grained manipulation, web-based interfaces expose a promising direction. These models can now perform primitive forms of spatial reasoning—such as cropping, rotating, or focusing on specific image regions—when prompted appropriately.

To quantify this capability, we conducted a pilot study on 100 clinical examples using the GPT–4o web interface. While accuracy did not dramatically improve, these interactions reveal early signs of visual reasoning traces—e.g., comparing lesion locations before making conclusions, highlighting suspicious zones, or identifying asymmetries through transformation.

Although not yet production-ready, this behavior suggests a conceptual convergence between VLMs and agentic image interpreters. Future benchmarks should consider such workflows, where models combine general reasoning with image manipulation tools in stepwise, verifiable fashion.



==> arxiv2510/sections_v0/capacities.tex <==
\section{Enhanced Clinical Reasoning Through Visual Chain-of-Thought}
Models that think with medical images support a richer set of diagnostic strategies. Instead of working from a single snapshot, they can revisit and revise interpretations based on tool-guided visual updates.

This dynamic inspection loop is especially valuable for tasks involving subtle, small, or evolving findings—situations where static systems often fail.
\begin{table}[ht]
\centering
\caption{Clinical tasks supported by visual chain-of-thought reasoning.}
\begin{tabularx}{\textwidth}{@{}l X X@{}}
\toprule
\textbf{Task Type} & \textbf{Example Use Case} & \textbf{Enabled Capability} \\
\midrule
Oncology detection &
Brain tumor localization with MRI &
Delimit lesion borders; support staging assessment \\
\addlinespace
Temporal comparison &
Tracking lung nodules across CT timepoints &
Align priors; measure growth or shrinkage \\
\addlinespace
Multi-view validation &
Fracture review on PA and lateral X-rays &
Cross-reference structures across views \\
\addlinespace
Subtle finding detection &
Microcalcifications in mammograms &
Zoom + contrast enhance to reveal faint patterns \\
\addlinespace
Whole-slide navigation &
Metastasis screening in pathology slides &
Low-power sweep + targeted high-magnification view \\
\addlinespace
Protocol adherence &
FAST ultrasound in trauma settings &
Sequentially inspect views for full coverage \\
\bottomrule
\end{tabularx}
\end{table}


==> arxiv2510/sections_v0/cases.tex <==
\section{Illustrative Case Studies Across Medical Modalities}
We present representative clinical tasks that benefit from visual chain-of-thought reasoning. The table below summarizes reasoning actions and their impact across modalities. More detailed examples are provided in the Appendix.


==> arxiv2510/sections_v0/conclusion.tex <==
\section{Conclusion and Future Directions}
The introduction of visual reasoning marks a meaningful advancement in how models interact with medical images. By incorporating dynamic image manipulation—zooming, cropping, and re-inspecting—directly into the reasoning process, these models begin to approximate the iterative, hypothesis-driven workflows used by clinical experts.
As demonstrated through case studies, this capability expands the range of clinical tasks that can be addressed with greater transparency and contextual awareness. From subtle abnormality detection to multi-view correlation and temporal comparisons, the ability to “think with images” allows for contextual updates at each reasoning step and generates interpretable visual artifacts along the way.
At the same time, this new reasoning paradigm introduces distinct risks. Hallucinations may emerge not only in the final output, but throughout the reasoning process—resulting in imagined structures, unsupported spatial relationships, or confident but inaccurate conclusions. These errors are particularly challenging in medical contexts, where decision-making requires verifiable, image-grounded evidence.
Toward Benchmarking Visual Reasoning in Medicine
We are actively extending this report with initial benchmark evaluations, focusing on task-specific accuracy for multi-step visual prompts. These evaluations are designed to assess both the correctness of final answers and the fidelity of the model’s intermediate reasoning steps.
We are also exploring early methods to characterize hallucination frequency, particularly in settings involving ambiguous or degraded visual input. These results will be incorporated in a forthcoming update.
Future directions
Advancing visual reasoning in clinical practice will require further progress across modeling, evaluation, and interface design. Key areas include:
\begin{enumerate}[1.]
\item Developing benchmarks that evaluate reasoning fidelity and visual traceability
\item Designing model architectures that support visual verification and mid-chain correction
\item Representing uncertainty throughout visual and textual reasoning steps
\item Building clinician-facing tools for reviewing and validating visual reasoning chains
\end{enumerate}
Visual reasoning represents an opportunity to transition from static perception to interactive interpretation. With careful validation and responsible deployment, it may serve as a foundation for more transparent, flexible, and clinically aligned systems for image-based decision support


==> arxiv2510/sections_v0/definition.tex <==
% \section{From Static Perception to Thinking with Medical Images}\label{sec2}

% Thinking with medical images introduces a new way of integrating perception and inference: models now engage with images iteratively during the reasoning process, rather than relying solely on a fixed initial visual representation.

% In earlier approaches, image understanding typically occurred in a single step: the system extracted a summary representation of the image, and subsequent reasoning operated only on this representation alongside the text. This resembles a radiology resident interpreting a scan after one initial pass—without the ability to revisit or re-examine specific regions in response to new questions.

% Thinking with medical images enables models to dynamically manipulate the image—zooming, cropping, rotating, enhancing—while forming conclusions. This process mirrors how experienced clinicians work: they may repeatedly inspect specific structures, compare regions, and update their assessments as new contextual information emerges. This active, visual chain-of-thought allows for higher sensitivity to subtle findings, improved reasoning transparency, and the potential for more interpretable outputs in diagnostic tasks.

% In the context of medical image interpretation, this change offers important new capabilities—especially in tasks that require fine-grained visual discrimination, multi-step reasoning, or contextual re-evaluation of ambiguous findings.

% \begin{table}[ht]
% \centering
% \caption{Core differences between one-shot interpretation and thinking with medical images.}
% \begin{tabularx}{0.8\textwidth}{@{}l X X@{}}
% \toprule
% \textbf{Aspect} & \textbf{One-shot Interpretation} & \textbf{Thinking with Medical Images} \\
% \midrule
% Visual input usage &
% Image seen once at the start; no interaction &
% Image re-inspected dynamically during reasoning \\
% \addlinespace
% Reasoning structure &
% All steps occur in text after initial inspection &
% Image and text steps interleave throughout \\
% \addlinespace
% Resolving ambiguity &
% Cannot revisit unclear areas &
% Uses zoom/crop/enhance to clarify findings \\
% \addlinespace
% Correction of errors &
% Early mistakes persist through reasoning &
% Intermediate steps allow visual correction \\
% \addlinespace
% Interpretability &
% Only final answer shown; reasoning is hidden &
% Each visual step and decision is observable \\
% \addlinespace
% Clinical analogy &
% Resident gives first-pass read from memory &
% Attending reevaluates image as needed \\
% \bottomrule
% \end{tabularx}
% \end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\textwidth]{figures/fig1.pdf}
% \caption{todo: makae it clear for clinician audience. adding model inference difference. Thinking with medical images: comparison of reasoning paradigms.
% a, In prior approaches, the model inspects the medical image once and generates a response using text-only reasoning, without revisiting the visual input.
% b, GPT o3-style models incorporate visual transformations such as crop, zoom, rotate, and enhance within their reasoning chain, enabling iterative image interpretation and intermediate verification steps. This allows for image-grounded, interpretable inference aligned with expert clinical workflows.
% }\label{fig1}
% \end{figure}

\section{What Does It Mean to Think with Medical Images?}

Recent advances in multimodal foundation models have expanded what AI systems can \textit{see} in medical data---but not necessarily what they can \textit{understand}. Today’s models can detect abnormalities, generate image captions, or answer visual questions. However, true clinical reasoning involves more than perception or pattern recognition. It requires the ability to \textbf{think with medical images}---a process that is inherently multimodal, contextual, and decision-oriented.

We define \textbf{thinking with medical images} as the capacity of an AI system to perform \textit{multistep, context-aware, and verifiable reasoning over both visual and textual clinical data}. This involves not only identifying and describing findings within images, but interpreting their significance in light of prior imaging, associated reports, clinical history, and laboratory results. It also involves generating interpretable hypotheses, managing uncertainty, and linking insights to downstream clinical decisions.

\subsection{From Perception to Multimodal Clinical Reasoning}

Much of the recent success in medical imaging AI has focused on \textit{perceptual tasks}: localizing lesions, classifying scan types, or generating reports. These tasks, while important, capture only a subset of what clinicians actually do. In practice, visual interpretation is always embedded within a broader clinical narrative that includes patient history, previous imaging, symptom trajectories, and diagnostic uncertainty.

Consider a radiologist reviewing a chest CT:
\begin{itemize}
    \item They do not simply report ``a new mass in the right upper lobe.''
    \item Instead, they compare it to prior scans, assess growth, consider the patient's smoking history and symptom onset, and often conclude with a differential diagnosis and management suggestion.
\end{itemize}

Similarly, an oncologist may examine imaging results in conjunction with biopsy findings and lab values, evaluating not just whether a lesion is present, but whether it represents progression, pseudoprogression, or treatment response.

Today’s benchmarks and models often fail to capture this \textbf{integrative reasoning process}. They reward shallow recall or generation rather than stepwise clinical logic. Most importantly, they treat perception and reasoning as separate stages, ignoring the fact that \textit{clinical understanding emerges from the continuous interplay between seeing, reading, comparing, and deciding}.

\subsection{A Capability Taxonomy: Core Components of Thinking with Medical Images}

To formalize what constitutes \textit{thinking with medical images}, we propose a taxonomy of core capabilities. These dimensions go beyond perception and encompass the multimodal reasoning tasks expected of AI systems aspiring to support clinical decision-making.

\begin{table}[h]
\centering
\caption{Core capabilities of thinking with medical images.}
\begin{tabular}{p{3.8cm} p{5.2cm} p{5.2cm}}
\toprule
\textbf{Capability} & \textbf{Description} & \textbf{Clinical Example} \\
\midrule
\textbf{Perceptual grounding} & Identify and localize clinically relevant features in an image & Detect right lower lobe opacity on chest X-ray \\
\textbf{Contextual inference} & Integrate findings with prior imaging, notes, and labs & Compare tumor dimensions over time; adjust interpretation based on infection markers \\
\textbf{Visual chain-of-thought reasoning} & Generate stepwise, interpretable logic grounded in both image and text & ``Focal opacity + fever + elevated CRP $\rightarrow$ pneumonia likely'' \\
\textbf{Uncertainty expression} & Identify ambiguous findings and communicate diagnostic uncertainty & Indeterminate pulmonary nodule in dense tissue; recommend follow-up CT \\
\textbf{Decision impact mapping} & Link visual and textual synthesis to concrete next steps & From lesion growth + new symptoms $\rightarrow$ recommend biopsy or treatment escalation \\
\bottomrule
\end{tabular}
\end{table}

This taxonomy can serve both as a \textit{design guide} for future models and as a \textit{framework for evaluation}---enabling researchers to assess progress not just in narrow tasks, but in holistic reasoning performance.

\subsection{Why This Matters for Real-World Clinical AI}

Clinical errors are rarely due to simple visual misses. Instead, they most often arise from \textit{misinterpretation}, \textit{failure to integrate information}, or \textit{overconfidence in ambiguous findings}. A model that can correctly detect an image feature but fails to place it in proper clinical context---or cannot express when it is uncertain---may propagate errors downstream with serious consequences.

Without the ability to reason through images in context, AI systems risk becoming advanced captioners or pattern matchers, rather than safe and trustworthy collaborators in care. Moreover, as AI is increasingly deployed in longitudinal workflows (e.g., tumor boards, radiology triage, diagnostic support), the absence of verifiable, multimodal reasoning capabilities becomes a barrier to real-world adoption.

If we seek to build foundation models that are not only capable but \textbf{clinically aligned}, then \textit{thinking with medical images}---understood as multimodal, interpretable, and verifiable reasoning---must be elevated as a central evaluation target.


==> arxiv2510/sections_v0/gap.tex <==
\section{Benchmark Landscape and Gaps}

Despite rapid advances in multimodal foundation models, the development and evaluation of Health AI systems remain dominated by benchmarks that do not reflect the complexity of real-world clinical reasoning—especially when medical images are involved. Existing benchmarks typically fall into two broad categories: \textit{text-dominant} and \textit{image-dominant}. While each has contributed to measurable progress, both categories fall short of evaluating whether models can truly reason with medical images in realistic clinical settings.

\subsection{Text-Dominant Benchmarks: High Performance, Low Fidelity}

Language-only benchmarks such as \textsc{MedQA}, \textsc{PubMedQA}, \textsc{HealthBench}, and \textsc{Med-Helm} are widely used to evaluate medical language models. These datasets often include multiple-choice questions derived from board exams, structured tasks drawn from electronic health records, or synthetic QA tasks constructed from clinical ontologies.

While effective at assessing factual knowledge and language-based reasoning, these benchmarks suffer from two core limitations:
\begin{itemize}
    \item \textbf{They assume structured, perceptual-free inputs.} Many tasks are text-only and assume that the relevant visual findings (e.g., from imaging) have already been correctly extracted and summarized.
    \item \textbf{They do not test visual understanding.} Models are not required to interpret or integrate visual data, leading to blind spots in evaluating perceptual reasoning and visual uncertainty.
\end{itemize}

As a result, models may appear clinically competent based on benchmark performance, while lacking any capacity to reason about visual evidence—the very signal that drives diagnostic decision-making in many clinical specialties.

\subsection{Image-Dominant Benchmarks: Narrow Tasks, Limited Reasoning}

Benchmarks such as \textsc{VQA-RAD}, \textsc{PathVQA}, \textsc{SLAKE}, \textsc{MedICaT}, and \textsc{CXR-Gen} introduce visual components to the evaluation pipeline. These datasets focus on tasks such as visual question answering, single-image report generation, or image-text retrieval.

Although these benchmarks help quantify performance on image-related tasks, they are limited in the following ways:
\begin{itemize}
    \item \textbf{They emphasize shallow, single-turn tasks.} Most focus on short, factoid-style questions without requiring reasoning across time, modality, or clinical context.
    \item \textbf{They lack temporality and multimodality.} Few benchmarks include comparisons across prior imaging, integration of clinical notes, or lab data—all essential for real-world clinical reasoning.
    \item \textbf{They do not evaluate reasoning quality.} Metrics such as BLEU, ROUGE, or simple QA accuracy fail to assess whether the model's inference path is clinically plausible or verifiable.
\end{itemize}

Consequently, even high scores on these benchmarks may hide brittle performance, hallucinations, or failures in contextual reasoning.

\subsection{A Conceptual Landscape of Benchmarks}

To better understand the coverage and limitations of current benchmarks, we position representative datasets within a two-dimensional space defined by:
\begin{itemize}
    \item \textbf{Y-axis: Reasoning Depth} — ranging from shallow label prediction to stepwise, multimodal reasoning.
    \item \textbf{X-axis: Multimodal Clinical Fidelity} — representing how well the benchmark reflects integrated, image-text clinical workflows.
\end{itemize}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{benchmark_landscape.pdf}
    \caption{\textbf{Benchmark coverage of reasoning and multimodal clinical fidelity in Health AI.} Each benchmark is plotted according to the depth of reasoning it requires (y-axis) and its fidelity to real-world multimodal clinical workflows (x-axis). Most benchmarks cluster in the lower-left quadrant, reflecting shallow reasoning over isolated modalities. Our proposed framework, \textsc{ThinkMedBench}, aims to shift evaluation toward the upper-right—capturing complex, agentic, and clinically grounded reasoning.}
    \label{fig:benchmark_landscape}
\end{figure}

As shown in Figure~\ref{fig:benchmark_landscape}, most widely used benchmarks cluster in the bottom-left quadrant—representing tasks that require neither deep reasoning nor realistic integration of image and text. \textsc{MedQA} and \textsc{HealthBench} exhibit high reasoning complexity but remain purely textual. Meanwhile, image-based datasets like \textsc{VQA-RAD} or \textsc{PathVQA} include visual inputs but require only shallow fact extraction.

No existing benchmark systematically evaluates the chain of reasoning that connects perception (e.g., image findings) with context (e.g., prior reports, clinical notes) and consequence (e.g., decision impact or uncertainty expression). Without such capabilities, model evaluation remains disconnected from real clinical utility.

\subsection{Summary: The Benchmark-Reality Gap}

Together, these limitations point to a critical gap in the development of Health AI systems. Current benchmarks measure isolated capabilities—retrieval, captioning, classification—but fail to test whether models can perform the type of visual, multimodal, and verifiable reasoning that clinicians rely on. This disconnect not only overestimates model readiness but also risks incentivizing brittle, hallucination-prone behaviors.

In the absence of benchmarks that reflect full clinical workflows, uncertainty handling, and perceptual integration, progress in Health AI risks being optimized for leaderboard performance rather than patient safety. Addressing this gap is essential for building systems that can not only perceive but also \textit{think with medical images}.


==> arxiv2510/sections_v0/hallucination.tex <==
\section{Imagined Steps, Real Risks: Visual Hallucinations in Medical Tasks}
\label{sec:hallucination_risks}

While “thinking with medical images’’ enables powerful new capabilities, it also introduces novel failure modes—most notably, \emph{hallucinations embedded within the reasoning process itself}.  
These errors go beyond traditional misclassifications: they arise when the model fabricates intermediate visual steps (e.g.\ cropping into nonexistent structures) and then builds confident conclusions on that false groundwork.

\medskip
\textbf{Figure (to be inserted).}  
Example hallucination chain: \emph{Prompt $\rightarrow$ visual‑tool sequence (zoom, crop) $\rightarrow$ fabricated intermediate $\rightarrow$ final answer $\rightarrow$ expert annotation of inconsistency}.

\subsection{Structural Limitations Underpinning Hallucinations}
\label{subsec:structural_limitations}

Our evaluation identifies three system‑level defects that together account for \TODO{\% of clinically significant errors} across \TODO{N total prompts} spanning radiology, pathology, and natural‑image tasks.

\begin{enumerate}[L1.]
    \item \textbf{Cascade hallucination / failure to converge.}  
    The model fail in (median X attempts) and respond... still‑incorrect hypothesis with high confidence instead of declaring uncertainty.  
    \emph{Triggers:} \TODO{N\_cascade} cases (\TODO{\%}) with median retries 4 (IQR 3–5).

    \item \textbf{Low self‑consistency.}  
    Identical inputs yield divergent reasoning paths and answers; mean pairwise agreement is only \TODO{\%} (\TODO{\%} for localisation tasks).  

    \item \textbf{Restricted in‑context visual operations.}  
    Only basic filters (thresholding, Canny, coarse crop/zoom, histogram equalisation) are callable;   
   
\end{enumerate}

\subsection{Observable Failure Behaviours and Clinical Risks}
\label{subsec:behaviour_patterns}

Table \ref{tab:behavioural_patterns} catalogues the \emph{observable} hallucination patterns encountered in practice and maps each to the \emph{structural limitation(s)} from Section~\ref{subsec:structural_limitations}.  
This mapping makes clear how a single architectural flaw can manifest as multiple clinically relevant error modes.


\medskip

\textbf{Figure (to be inserted):} \\
An example hallucination chain: Prompt $\rightarrow$ visual tool sequence (zoom, crop) $\rightarrow$ fabricated intermediate $\rightarrow$ final output $\rightarrow$ expert annotation of inconsistency

\medskip

\begin{table}[ht]
\centering
\caption{Common patterns of hallucinated visual reasoning and associated clinical risks.}
\begin{tabularx}{\textwidth}{@{}l X X@{}}
\toprule
\textbf{Type} & \textbf{Example Behavior} & \textbf{Clinical Risk} \\
\midrule
Fabricated visual region & Zooms or crops into areas without relevant content & Invents findings (e.g., ``nodule'' that does not exist) \\
False temporal inference & Claims growth or shrinkage across serial images without alignment & Misguides treatment; risks overtreatment or missed change \\
Overinterpretation of noise & Interprets compression or artifacts as pathology & Misdiagnosis on low-quality scans \\
Redundant reasoning loops & Repeats tools to simulate depth or inspection rigor & Creates a false impression of clinical thoroughness \\
Confident but incorrect & Generates well-reasoned yet ungrounded conclusions & Hard to detect; erodes trust in automated outputs \\
\bottomrule
\end{tabularx}
\end{table}

\medskip

These errors are particularly insidious because they are often \textit{internally coherent}: the model's reasoning appears logical and plausible, even when its underlying visual assumptions are false. This issue likely stems not from the model’s perceptual capacity, but from how it has been trained—rewarding coherent step-by-step explanations, even when those explanations are not grounded in the image.

As a result, hallucinations can be confident, fluent, and dangerously persuasive—a serious concern for clinical settings that demand verifiable, image-based evidence.

\subsection*{Mitigation Strategies}

To safely deploy visual reasoning models in high-stakes environments, several safeguards are essential:
\begin{enumerate}[1.]
\item Develop hallucination-aware benchmarks that penalize plausible but unsupported visual chains
\item Track tool usage to ensure visual steps are traceable and grounded in actual image regions
\item Incorporate uncertainty-aware reasoning chains, including self-check and abort mechanisms
\item Enable external review of intermediate steps, particularly in workflows involving medical risk
\end{enumerate}


==> arxiv2510/sections_v1/analysis.tex <==
\section{Rethinking Evaluation: Benchmark Flaws and Emergent Model Behaviors}

Despite rising accuracy across individual benchmarks, our analysis uncovers systematic limitations in both the design of current benchmarks and the interpretation of model performance. We distill several key findings that challenge common assumptions and highlight the need for a more grounded, clinically aligned evaluation paradigm.

\subsection{Benchmarks Claim Multimodality but Are Text-Resolvable}

While many benchmarks are framed as multimodal tasks, in practice they are often solvable using text alone. JAMA Clinical Challenge, for example, yields higher accuracy with text-only inputs than with full image-text multimodal settings—suggesting that visual inputs may introduce noise or be disregarded by the model. This undermines the benchmark’s ability to test perceptual understanding and questions its utility for evaluating visual reasoning.

\subsection{Supposedly Similar Benchmarks Yield Divergent Model Behaviors}

Benchmarks designed to assess similar reasoning capabilities often yield drastically different outcomes on the same model. GPT-o3-zero, for instance, achieves over 86\% on JAMA but drops to 67\% on NEJM when using the same text-only setup. This inconsistency reveals that benchmarks vary not only in difficulty, but also in structural assumptions—such as phrasing templates, task framing, or content filtering—which influence model performance in unpredictable ways.

\subsection{Emergent Capabilities Remain Undetected by Existing Benchmarks}

Recent frontier models exhibit capabilities—such as spatial grounding, longitudinal comparison, and uncertainty hedging—that are not captured by current benchmark metrics. Our case studies with GPT-o3’s image editing features reveal stepwise reasoning chains involving crop, rotate, and compare actions. Yet, standard benchmarks lack instrumentation to detect or reward such behaviors, highlighting a mismatch between what models are capable of and what evaluations measure.

\subsection{Benchmark Construction Risks Pretraining and Train-Test Leakage}
% \Aiden{Flora to review}
We observe several signals suggesting the presence of pretraining leakage or content overlap. Gemini-2.5-pro performs surprisingly well on certain benchmarks in text-only settings, raising concerns about memorization rather than reasoning. Moreover, many public benchmarks source questions from published articles, textbooks, or open forums—some of which are known to be present in the pretraining corpora of large models. Without audit trails or provenance tracking, it becomes difficult to disentangle true generalization from exposure.
\Aiden{add exp: add perturb to input text e.g. unit/number, and test gemini/gpt o3 on text only settup }
\subsection{Poor Generalization Between Benchmarks Limits Robustness}
% \Aiden{Flora to review }
% Models trained on one benchmark often fail to generalize to structurally similar benchmarks. In prior work on OmniMedVQA, we found that training VLMs on large-scale cross-modal datasets did not improve performance on MMMU-Pro-Health, despite overlapping modalities and question types. This points to significant domain and format-specific overfitting, and suggests that current benchmarks are narrow tests rather than general diagnostic tools.

Models trained on one benchmark often fail to generalize to structurally similar benchmarks. We conducted a pilot study and train a VLM starting from Qwen2.5-VL-7B-Instruct model on 80\% randomly split OmniMedVQA via GRPO reinforcement learning (can cite x-reasoner and med-r1 here). We found the outcome VLM can significantly increase performance on the in-distribution OmniMedVQA testset (from 57\% to 97\% accuracy), however it hurts performance other multimodal VQA tasks such as MMMU-Pro-Health (from 34\% to 29\% accuracy), despite overlapping modalities and question types. This points to significant domain and format-specific overfitting, and suggests that current benchmarks are narrow tests rather than general diagnostic tools.

\subsection{Reasoning and Visual Complexity Vary Even Within a Benchmark}

Many benchmarks span a wide range of difficulty and modality alignment within the same dataset. In OmniMedVQA, for example, questions vary from low-complexity image captions to high-complexity, multi-modal inference tasks involving pathology slides. This internal heterogeneity complicates training, as models are simultaneously expected to learn simple mappings and sophisticated reasoning within a single objective—resulting in brittle generalization and incoherent optimization.

% \subsection{Summary}

% Together, these findings suggest that benchmark performance alone is a poor proxy for generalizable reasoning or clinical utility. The current paradigm overstates model capabilities, under-represents failure modes, and overlooks emergent reasoning behavior. A reevaluation of benchmark design is urgently needed—one that explicitly measures verifiability, perceptual alignment, reasoning depth, and generalization across tasks and modalities.


==> arxiv2510/sections_v1/intro_2.tex <==
\section{Introduction}
\label{sec:intro}

Large language models (LLMs) and Large multi-modality models (LMMs) are rapidly gaining traction in healthcare for their ability to encode vast clinical knowledge and reason through complex inputs. If harnessed correctly, LLMs could help bridge gaps in health information access and decision support, but realizing this potential requires that such models perform reliably and safely in the diverse, high-stakes situations of clinical practice. To that end, rigorous evaluation has become essential – shared benchmarks serve as key indicators of progress – yet current evaluation practices in health AI remain insufficient and limited. 

One major limitation is a lack of clinical realism in how we test LLMs. Many are based on idealized multiple-choice medical exam questions or structured factoid queries that assume inputs are already interpreted and clean. For example, standardized exam datasets typically present idealized vignettes rather than messy electronic health records with ambiguities and domain-specific shorthand; indeed, only about 5\% of LLM evaluations to date incorporate any real clinical data such as actual EHR notes. These narrowly scoped evaluations often allow models to perform well through pattern recognition or memorization, without truly testing the contextual understanding and iterative reasoning required in practice. Furthermore, many benchmarks have not been validated against expert physician judgment, calling into question whether high scores correspond to clinically acceptable performance. 

These shortcomings have created a clear gap between benchmark performance and real-world utility. The most powerful LLMs can now achieve high scores on medical licensing exams,  these accomplishments inadequately capture the complexity and nuance of real-world clinical decision-making.. Models excelling at simplified benchmarks may still falter when confronted with the nuances of genuine patient cases – for instance, synthesizing information from an unstructured clinical note or responding to an evolving multi-turn dialogue with a patient. 

Recent datasets begin to address isolated pieces of the problem. HealthBench emphasizes open-ended physician-patient interactions, while Med-HELM introduces a task taxonomy covering dozens of use cases. However, both remain text-centric, excluding visual reasoning from images—a critical component in many domains such as radiology, dermatology, and pathology. Also, there is a pressing need for development of both patient-facing tools that enhance accessibility and engagement, and clinician-facing systems that support diagnostic reasoning, documentation, and decision-making in real-world settings. An evaluation paradigm that accounts for these roles across the continuum of care is also a critical priority.
Despite these advances, significant gaps remain. Each of the current benchmarks tends to address only pieces of the puzzle – for instance, HealthBench focuses on open-ended text conversations but covers a limited range of tasks, whereas MedHELM covers many tasks but primarily within textual contexts. No single framework yet integrates all the crucial dimensions required for a truly faithful assessment of an LLM’s clinical utility.

% We close this gap with a unified evaluation framework that integrates three missing dimensions:
% \begin{enumerate}
%     \item \textbf{Reasoning complexity}: Tests multi-step clinical reasoning instead of one-shot Q\&A, mirroring the nuanced decision-making in patient care.
%     \item \textbf{Visual dependency}: Adds tasks that require interpreting radiology, pathology, and other clinical images—content missing from text-only benchmarks.
%     \item \textbf{Clinical realism}: Grounds all evaluations in authentic case distributions and workflows so results reflect real-world performance, not sanitized inputs.
% \end{enumerate}
In this paper, we revisit how we evaluate foundation models in health AI. We argue that the field urgently needs a principled framework to assess what benchmarks actually test, how they differ in complexity, and how models behave across them. To better understand these disconnects, we ask: what are today’s health benchmarks actually measuring, and how do they align with real clinical needs? We contribute:

\begin{enumerate}
    \item \textbf{Benchmark the benchmarks:} We curate and re-analyze widely used benchmarks using a structured rubric that scores reasoning complexity and visual dependency—validated through clinician review.
    \item \textbf{Reveal model-behavior mismatches:} We show how performance varies across tasks and modalities, exposing spurious multimodal degradation, lack of reasoning robustness, and poor transfer between benchmarks.
    \item \textbf{Propose actionable design principles:} We distill our findings into recommendations for future benchmarks—emphasizing clinical context, verifiable inference, and alignment with real-world workflows.
\end{enumerate}
% By bringing these pillars into a single, principled benchmark, we align evaluation with real-world requirements and provide clear guidance for developing safer, more effective health-AI systems.
% Our framework unifies reasoning and vision under clinically grounded evaluation. 
By doing so, we hope to realign benchmark development with practical clinical utility—moving from leaderboard chasing to trustworthy, verifiable, and useful health AI systems.

==> arxiv2510/sections_v1/introduction.tex <==
% \section{Introduction}
% This paper aims to define, benchmark, and evaluate the clinical utility of visual chain-of-thought reasoning with medical images. While prior work has focused on answer accuracy in constrained tasks (e.g., VQA multiple choice), we focus on scenarios where answering a question requires explicit, stepwise visual reasoning, similar to what a physician would do during image interpretation.

% We are collaborating with domain experts (starting with radiologists) to:

% Define task-specific reasoning criteria and evaluation metrics

% Curate benchmark datasets where correct answers require visual inspection + transformation, not just global cues or shortcut artifacts

% Evaluate state-of-the-art models not just on final answer correctness, but on the faithfulness and traceability of their reasoning steps

% Our goal is twofold: (1) provide a scientifically grounded benchmark for evaluating medical visual reasoning, and (2) explore how interpretable, tool-assisted reasoning chains can facilitate future model training, mitigate hallucinations, and integrate more naturally into clinical workflows.

% Ultimately, this work is a step toward clinically aligned, explainable AI systems that reason in a way physicians can inspect, trust, and potentially learn from
% Recent advances in multimodal foundation models have enabled unprecedented progress in medical image understanding. However, most existing systems treat the visual modality as a one-time input: an image is processed once to extract a fixed representation, which is then used for downstream reasoning. This static approach limits the model's ability to resolve uncertainty, revise interpretations, or inspect ambiguous findings.

% GPT o3 and o4 models introduce a new reasoning paradigm: they can \textit{think with images} by interleaving visual transformations—such as cropping, zooming, rotating, and enhancing—within the chain-of-thought reasoning process. This enables the model to dynamically engage with the image, refine its interpretation, and expose intermediate visual steps.

% In this report, we provide an early technical and clinical characterization of this capability. We compare it to prior paradigms, describe its new diagnostic affordances, illustrate case studies across modalities, and highlight important failure modes, including visual hallucinations. We close with directions for benchmarking and safe deployment.

% Recent advances in large foundation models have driven impressive progress in health AI. General-purpose large language models now surpass human performance on medical exams, while domain-specific vision-language models (VLMs) excel in tasks like visual question answering (VQA) and radiology report generation.

% Yet, current benchmarks are either saturated by SOTA models or fail to reflect real clinical workflows. Most assume that images have been correctly interpreted—overlooking the fact that critical errors often originate in upstream visual understanding. These upstream errors propagate through clinical reasoning, remaining undetectable by downstream tasks alone.

% Recent textual benchmarks (e.g., HealthBench, Med-Helm) focus predominantly on textual reasoning and structured clinical inference, effectively decoupling decision-making from its visual foundations. Conversely, visual benchmarks prioritize isolated image recognition, neglecting multi-step, context-rich clinical reasoning. Consequently, even models with demonstrated reasoning capacity are not verifiably tested in realistic, end-to-end scenarios.

% We argue that the frontier of health AI lies in thinking with medical images: integrating visual evidence, patient context, and clinical reasoning through explicit, verifiable inference steps. Emerging capabilities, such as GPT-o3’s real-time image manipulation and multimodal reasoning or recent healthcare agent frameworks, underscore this direction, but existing evaluation methods have yet to catch up.
% In this paper, we:
% \begin{itemize}
%     % \item Analyze benchmark-task gaps across reasoning complexity and visual dependence
    
%     % \item Reveal failure patterns from recent frontier models (GPT-o3, GPT-o4 mini,, Gemini 2.5 pro, LLaVA-Med, etc.)
    
%     % \item Highlight the importance of verifiable, context-aware visual reasoning
    
%     % \item Propose next-generation benchmark principles grounded in real-world clinical workflows
% \end{itemize}
% By critically revisiting what we measure, we aim to accelerate progress toward clinically trustworthy and practically impactful health AI.

\section{Introduction}

Despite rapid progress in large foundation models, today’s health AI ecosystem is bottlenecked—not by a lack of capable models, but by benchmarks that fail to reflect clinical reality.

General-purpose large language models (LLMs) now surpass human performance on medical exams, and vision-language models (VLMs) achieve strong results on tasks like medical VQA and radiology report generation. Yet these gains offer a false sense of progress—driven by benchmarks that are either saturated or structurally divorced from clinical workflows.

On one side, researchers are forced to optimize for benchmark performance—chasing leaderboards rather than clinical utility. Models overfit to narrow test sets, exploit spurious cues, or memorize shallow correlations while receiving inflated scores. On the other side, healthcare practitioners seeking trustworthy AI find little alignment between benchmark claims and real-world needs. This disconnect stems from foundational flaws in how we evaluate.

Most benchmarks assume perfect image understanding, effectively skipping the most error-prone part of clinical interpretation. Others isolate vision from reasoning, or compress complex tasks into multiple-choice formats that fail to test inference depth, context integration, or verifiability. Recent textual benchmarks (e.g., HealthBench, Med-Helm) lean heavily on structured inputs, while visual tasks reduce perception to short-form recognition. In effect, we fail to measure what matters most: the ability to think with medical images.

This paper takes a step back. We argue that the health AI community urgently needs a \emph{benchmark of benchmarks}—a structured framework to assess what current evaluations actually measure, what they miss, and how they align (or misalign) with clinical needs. We propose a new lens for evaluating health benchmarks based on two critical dimensions: reasoning complexity and visual dependency. Using these axes, we reclassify widely-used tasks, engage clinicians to score them, and systematically analyze how frontier models behave under these conditions.

\subsection*{Contributions}

Our contributions are four-fold:

\begin{enumerate}
    \item \textbf{Benchmark the benchmarks:} We analyze reasoning complexity and visual dependence across widely used health AI benchmarks, exposing how many fail to reflect the demands of real-world clinical decision-making.

    \item \textbf{Reveal model and benchmark failure patterns:} Through systematic evaluation of frontier models, we show how performance varies inconsistently across benchmarks, uncovering issues like reasoning instability, spurious multimodal degradation, and lack of generalization across tasks.

    \item \textbf{Establish a clinically grounded evaluation rubric:} We design a rubric capturing reasoning and visual complexity, validated through clinician annotation. This scoring framework enables principled benchmark comparison and composite model evaluation aligned with clinical relevance.

    \item \textbf{Propose actionable design principles:} We outline practical recommendations for building next-generation benchmarks that incorporate clinical context, support multi-step reasoning, penalize unverified outputs, and better reflect real-world healthcare workflows.
\end{enumerate}


==> arxiv2510/sections_v1/limitation.tex <==
\section{Limitations and Discussion}
\textbf{Benchmark Scope and Task Coverage}
While our rubric spans key dimensions of reasoning and visual complexity, the selected benchmarks do not exhaust the full spectrum of clinical tasks. Domains such as mental health, genomics, and patient-facing communication remain underexplored. Our focus has also been on VQA and report generation tasks, which—though highly impactful—represent a subset of real-world decision support scenarios.

\noindent \textbf{Clinician Annotations and Subjectivity}
Despite calibrating scores across multiple expert annotators, the rubric-based ratings (e.g., visual dependency, reasoning complexity) inevitably carry a degree of subjectivity. While inter-rater agreement was moderate to strong, future work should explore more granular, consensus-driven schema and involve a broader pool of annotators across specialties.

\noindent \textbf{Evolving Model Capabilities}
Rapid improvements in foundation models may quickly shift what is considered challenging. Benchmarks must be continuously updated to reflect evolving capabilities and avoid saturation. Our framework is designed to accommodate this dynamism, but the specific benchmark scores presented here may become outdated.

\noindent\textbf{Limitations in Diagnostic Ground Truth}
For report generation, we address the limitations of using radiology reports as gold standards, yet even our clinician-annotated pilot inherits constraints. Disagreement among experts, ambiguity in clinical images, and variability in institutional norms are all sources of noise that can affect evaluation fidelity.

\noindent \textbf{Discussion: Toward Benchmark–Model Co-Design}
Our findings suggest that benchmarks should not only evaluate models, but also inform their design. Preliminary trends indicate that multi-task training and modality-aware architectures may generalize better across tasks with high reasoning demands. We believe future work should more tightly couple benchmark development with architectural exploration—an avenue we are pursuing through our upcoming benchmark release.

==> arxiv2510/sections_v1/method.tex <==
\section{Repositioning Health Benchmarks} \label{sec:benchmark_repositioning}
\subsection{Benchmark Selection}

Despite widespread adoption, current benchmarks in health AI rarely reflect the reasoning processes or visual demands encountered in real-world clinical workflows. Many have become saturated with near-ceiling performance from state-of-the-art models, yet still fail to expose critical failure modes.

To systematically assess what today’s benchmarks measure—and what they miss—we select a representative set of widely used tasks spanning different input modalities, interaction formats, and levels of clinical abstraction. These include single-modality visual QA (e.g., VQA-RAD), cross-modality grounded QA (e.g., PMC-VQA, OmniMedVQA), clinically grounded case reasoning (e.g., JAMA Clinical Challenge, NEJM Case Reports), and open-ended generation tasks (e.g., MIMIC-CXR).

Our goal is not merely to compare accuracy across tasks, but to situate each benchmark along two critical axes: \textbf{reasoning complexity} and \textbf{visual dependency}—dimensions that together determine how well a benchmark reflects real clinical decision-making.


% \begin{itemize}
%     \item \textbf{VQA-RAD}: Single-image, factoid-style QA (e.g., “Is there a mass?”). Tasks are shallow, with minimal clinical context and low visual complexity.
    
%     \item \textbf{PMC-VQA / OmniMedVQA}: Cross-modal VQA combining biomedical text and radiology images. Requires domain-specific knowledge, fine-grained visual understanding, and multi-hop reasoning.
    
%     \item \textbf{JAMA \& NEJM Clinical Challenges}: Case-based multiple-choice questions. JAMA items are typically solvable from text alone; NEJM requires visual interpretation, temporal comparison, and integration of clinical context. We treat them as a single task type—\textit{clinical case reasoning}—but score them separately based on visual complexity.
    
%     \item \textbf{MIMIC-CXR Report Generation}: Open-ended, free-text radiology report generation from chest X-rays. Demands accurate image grounding, comparison with prior studies, and clinically fluent narrative synthesis.
% \end{itemize}

% This benchmark set spans a wide range of clinical tasks—from structured question answering to complex, multimodal decision-making—and reveals where current models succeed or fall short under real-world constraints.

\subsection{Rubric for Reasoning and Visual Complexity}
We define reasoning complexity as the depth, structure, and ambiguity of inference required to arrive at a clinically sound response. Visual dependency captures the extent to which image understanding is essential to task completion, rather than auxiliary or irrelevant.

Each axis is composed of several clinically grounded sub-criteria (see Tables~\ref{tab:reasoning_criteria} and~\ref{tab:visual_criteria}) scored on a 3-point ordinal scale. This yields a principled framework to locate benchmarks within a 2D space—quantifying how visually dependent and cognitively demanding each task is.

\begin{table}[htbp]
\centering
\small
\begin{tabularx}{\textwidth}{l|X|X|X}
\toprule
\textbf{Category} & \textbf{1 (Low)} & \textbf{2 (Moderate)} & \textbf{3 (High)} \\
\midrule
\textbf{1. Reasoning Steps} & One-step (e.g., identify organ) & Combine findings (e.g., abnormality + location) & Differential diagnosis or staged inference \\
\textbf{2. Clinical Context} & No patient context needed & Some (e.g., age, complaint) & Full scenario (labs, history, clinical reasoning) \\
\textbf{3. Time/Sequence Info} & Not referenced & Sometimes referenced & Required (e.g., compare prior scans or progression) \\
\textbf{4. Uncertainty Handling} & No ambiguity & Some vagueness or ambiguity & Requires hedging, differentials, or multiple possibilities \\
\textbf{5. Decision Impact} & No impact (e.g., trivia) & Some impact (e.g., follow-up, triage) & High impact (e.g., diagnosis, treatment selection) \\
\bottomrule
\end{tabularx}
\caption{Rubric for scoring reasoning complexity across health AI benchmarks.}
\label{tab:reasoning_criteria}
\end{table}

\vspace{1em}

\begin{table}[htbp]
\centering
\small
\begin{tabularx}{\textwidth}{l|X|X|X}
\toprule
\textbf{Category} & \textbf{1 (Low)} & \textbf{2 (Moderate)} & \textbf{3 (High)} \\
\midrule
\textbf{1. Text-alone Solvable} & Yes, image unnecessary & Maybe, image adds context & No, image essential to answer correctly \\
\textbf{2. Visual Detail Needed} & Glance is enough & Moderate detail (e.g., detect a finding) & Expert-level detail (e.g., subtle lesion or measurement) \\
\textbf{3. Spatial Understanding} & Not needed & Region or side matters & Exact location or distribution is critical \\
\textbf{4. Image Quality Sensitivity} & Not sensitive to small changes & Somewhat sensitive & High sensitivity to subtle visual cues \\
\textbf{5. Multi-view / Temporal Alignment} & No comparison needed & Sometimes referenced & Must compare across views or timepoints \\
\bottomrule
\end{tabularx}
\caption{Rubric for scoring visual dependency across health AI benchmarks.}
\label{tab:visual_criteria}
\end{table}


% Current health AI leaderboards fail to capture what tasks truly demand. A model might top a benchmark while relying on pattern matching or shortcut heuristics. To uncover what lies beneath performance metrics, we introduce a structured rubric to score the inherent complexity of each benchmark along two clinically critical axes:

% \begin{itemize}
%     \item \textbf{Reasoning Complexity} — How much multi-step, uncertainty-aware clinical inference is required
%     \item \textbf{Visual Dependency} — How central accurate, expert-level image interpretation is to task success
% \end{itemize}

% The rubric was developed in consultation with three board-certified clinicians (radiology, internal medicine, pathology), who independently reviewed a representative subset of each benchmark and scored tasks from 1 (low) to 3 (high). Each axis consists of four key dimensions reflecting real-world decision-making demands.

% \paragraph{Reasoning Complexity Criteria}
% % Add to preamble:
% % \usepackage{booktabs}
% % \usepackage{float}

% \begin{table}[htbp]
% \centering
% \small
% \begin{tabularx}{\textwidth}{X | X | X | X}
% \toprule
% \textbf{Dimension} & \textbf{Low (1)} & \textbf{Moderate (2)} & \textbf{High (3)} \\
% \midrule
% Reasoning Steps & Factoid QA & Multi-step synthesis (e.g., findings + diagnosis) & Multi-phase inference, differentials \\
% Clinical Context & None/minimal & Partial context (e.g., age, complaint) & Full scenario integration \\
% Temporal/Longitudinal & Not required & Sometimes referenced & Required for correct reasoning \\
% Uncertainty Handling & Absent & Basic ambiguity/hedging & Differential diagnosis or uncertainty modeling \\
% \bottomrule
% \end{tabularx}
% \caption{Rubric for scoring reasoning complexity across health AI benchmarks.}
% \label{tab:reasoning_criteria}
% \end{table}

% \begin{table}[htbp]
% \centering
% \small
% \begin{tabularx}{\textwidth}{X | X | X | X}
% \toprule
% \textbf{Dimension} & \textbf{Low (1)} & \textbf{Moderate (2)} & \textbf{High (3)} \\
% \midrule
% Text-alone Solvable & Yes & Sometimes & No (image essential) \\
% Visual Detail Needed & Minimal & Moderate (e.g., lesion boundaries) & High (expert-level cues required) \\
% Spatial Reasoning & Not required & Moderate (e.g., side awareness) & Essential (anatomical localization) \\
% Image Quality Sensitivity & Low or none & Moderate impact & High sensitivity (subtle changes matter) \\
% \bottomrule
% \end{tabularx}
% \caption{Rubric for scoring visual dependency across health AI benchmarks.}
% \label{tab:visual_criteria}
% \end{table}

% \subsection{Complexity Profiles of Health AI Benchmarks}

% To empirically characterize the demands of current health AI benchmarks, we conducted a structured complexity assessment using the rubric defined in Section~\ref{sec:rubric}. Our goal was to quantify what each benchmark truly tests—beyond what leaderboard accuracy reveals.

% \subsubsection{Clinician Scoring Study Design}

% Three board-certified physicians (radiology, internal medicine, and pathology) independently reviewed representative examples from five benchmarks. Each example was scored across eight rubric dimensions—four for \textit{reasoning complexity} and four for \textit{visual dependency}. Scoring was performed on a 1–3 scale (low to high), and discrepancies were resolved through consensus discussion.

\subsection{Clinician Scoring Procedure}
To ensure that our benchmark repositioning reflects real-world clinical judgment, we employed a clinician-in-the-loop approach. Rather than inferring benchmark properties from task descriptions alone, we asked practicing clinicians to directly assess a representative subset of benchmark examples.

\textbf{Scoring Method.} Each clinician was presented with 30–50 examples per benchmark, randomly sampled to reflect task diversity. For each example, clinicians rated eight dimensions—four related to reasoning complexity (Table~\ref{tab:reasoning_criteria}) and four related to visual dependency (Table~\ref{tab:visual_criteria})—on a 3-point ordinal scale: low (1), moderate (2), or high (3). Definitions and example-based anchors were provided for each criterion to minimize ambiguity.

\textbf{Example-Based Evaluation.} Rather than rating entire benchmarks globally, clinicians scored individual examples to capture within-task variability. This design accounts for the fact that some benchmarks contain a wide mix of easy and difficult cases, or questions that vary in visual necessity. For each benchmark, we report the mean score across examples and raters on each axis, producing a robust and interpretable benchmark-level profile.

\textbf{Clinician Background.} Our annotators included board-certified physicians and senior clinical trainees (e.g., residents, fellows) with experience in diagnostic specialties such as radiology, internal medicine, and emergency medicine. All were blinded to model outputs and benchmark identity to prevent anchoring effects.

\textbf{Annotation Instructions.} Instructions emphasized evaluating clinical reasoning and image relevance as they would in real diagnostic decision-making. Rather than relying on the task’s stated modality or format, clinicians were asked: \emph{“To answer this question accurately and confidently, how much reasoning is required? How essential is the image?”} The full instruction set provided to annotators is included in Appendix~\ref{appendix:labeling}.

\textbf{Inter-rater Agreement and Aggregation.} Each example was scored independently by at least two clinicians. We observed high consistency across raters (Cohen’s $\kappa$ = \textit{[placeholder, to be added]}). Benchmark-level scores were aggregated by averaging across examples and raters, and visualized in the benchmark landscape (Figure~\ref{fig:benchmark_landscape}).

\textbf{Why Example-Level Scoring Matters.} Many existing meta-analyses assume that benchmark difficulty is uniform across items, leading to coarse or misleading assessments. Our method surfaces intra-task heterogeneity and avoids overgeneralization, yielding a more nuanced view of how benchmarks align with real clinical reasoning and perceptual demands.


% \begin{itemize}
%     \item \textbf{Sample Size:} 15–20 representative examples per benchmark
%     \item \textbf{Scoring Protocol:} Independent rating $\rightarrow$ Consensus discussion $\rightarrow$ Final average
%     \item \textbf{Aggregation:} Each benchmark’s final visual and reasoning score was computed as the mean of its four sub-dimension scores.
% \end{itemize}

% \subsubsection{Results Summary}

% Figure~\ref{fig:benchmark-map} plots benchmark positions in a 2D space:
% \begin{itemize}
%     \item \textbf{X-axis:} Average Visual Dependency Score
%     \item \textbf{Y-axis:} Average Reasoning Complexity Score
% \end{itemize}

% This benchmark map reveals a structured landscape of task demands:

% \begin{itemize}
%     \item \textbf{VQA-RAD:} Located in the bottom-left quadrant—low reasoning and visual complexity. Tasks are typically surface-level and factoid-based.
%     todo
%     % \item \textbf{PMC-VQA / OmniMedVQA:} Occupy the mid-region, requiring some cross-modal reasoning and domain knowledge, but with limited contextual depth.
%     % \item \textbf{JAMA and NEJM:} Cluster in the upper region of reasoning complexity. NEJM scores higher on visual dependency, while JAMA remains largely text-resolvable.
%     % \item \textbf{MIMIC-CXR:} Positioned in the top-right corner—demanding both high visual understanding and complex clinical synthesis.
% \end{itemize}

% \subsubsection{Main Insights}

% \begin{itemize}
%     \item Benchmark scores expose structural differences not captured by model accuracy alone.
%    \item \textbf{Text-solvable tasks} (e.g., JAMA) risk overestimating real-world model competence.
%     \item \textbf{High-complexity tasks} (e.g., NEJM, MIMIC-CXR) better reflect the multimodal, longitudinal, and ambiguous nature of clinical reasoning.
%     \item This mapping motivates \textit{next-generation evaluations} that explicitly test for both perceptual grounding and reasoning depth.
% \end{itemize}

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.7\textwidth]{figures/fig1.pdf}
    \includegraphics[width=0.85\textwidth]{figures/score_plot.png}
    \caption{PLACEHODER: Benchmark complexity landscape. Each benchmark is positioned using clinician-assessed average visual dependency (X-axis) and reasoning complexity (Y-axis). Real-world tasks (top-right) are underrepresented in current benchmarks.}
    \label{fig:benchmark_landscape}
\end{figure}

\subsection{Benchmark Classes}
To guide subsequent analysis, we categorize benchmarks into four broad classes:

\begin{itemize}
    \item \textbf{Single-Modality VQA:} e.g., VQA-RAD, consisting of short-form factoid questions grounded in radiographs.
    \item \textbf{Cross-Modality Grounded QA:} e.g., PMC-VQA, OmniMedVQA, which require integrating textual and visual information from biomedical literature or imaging.
    \item \textbf{Clinical Case Reasoning:} e.g., JAMA Clinical Challenge, NEJM Case Reports, focused on multi-step diagnostic inference with mixed or filtered image access.
    \item \textbf{Open-Ended Generation:} e.g., MIMIC-CXR report generation, where models must produce free-form, clinically coherent summaries with temporal and spatial reasoning.
\end{itemize}

These categories offer increasing coverage across the reasoning-visual spectrum. Yet, as we show in the next section, they also expose surprising inconsistencies in model performance and benchmark behavior—calling into question how well our current evaluation tools reflect real clinical capabilities.


==> arxiv2510/sections_v1/principle.tex <==
% \section{What to do}
% connect to medbench 
% 1. data contamination
% 2. chain of thought verifible 
% 3. 
% \Aiden{Ying to give bullet}
% A comparison of the $<$ model's training recipe and performance in our benchmark$>$ would provide the readers with helpful implications on how to improve their model in certain dimensions. This would be a valuable takeaway for our readers, as they would like to know ``how to solve the problems'' after being convinced in ``the problem we surfaced'' by our benchmark. Potential assumptions we may provide:
% \begin{itemize}
%     \item Is ``native multi-modality'' vs retrofitted multi-modality better for image-based reasoning
%     \item Does multi-task learning (e.g. combining VQA, report gen, etc.) improve one task (related to QRad - does QA improve reasoning, which is beneficial for report gen?)
%     \item With the same computation budget, shall we scale the image encoder or text decoder to improve text reasoning vs. image grounding capacity? Ideally, this one could be an experiment that trains several models, all with M+N = 12 layers transformer. Each model has a different M and N values, while the sum is always 12. This helps us to understand where shall we draw the line between the encoder and decoder.
%     \item Existing work uses different LR for the encoder and decoder. If encoder uses a larger LR, does it improve image grounding? If the decoder uses a larger LR, does it improve reasoning? If the module was pre-trained on a non-medical domain, does using a smaller LR transfer its reasoning/grounding capability?
% \end{itemize}

% \Aiden{while I'm writing this list, I feel these questions can only be addressed by proposing our method or train our own models, and answer these questions in ablation studies...}

% experiment design principle

\section{Designing Next-Generation Benchmarks for Health AI}
\label{sec:nextgen_benchmarks}

Based on our analysis, we propose four key principles to guide the development of next-generation health AI benchmarks:

\begin{enumerate}
    \item \textbf{Reflect end-to-end clinical workflows:} Evaluation should span the full diagnostic chain, from image perception to documentation and decision-making—not isolate subcomponents. Tasks should match how clinicians reason, revise, and communicate over time.
    
    \item \textbf{Reward interpretable and verifiable reasoning:} Rather than optimize for black-box accuracy, benchmarks should surface intermediate steps, allow error tracing, and encourage transparent justifications that align with expert judgment.
    
    \item \textbf{Capture multimodal dependencies:} Clinical intelligence often arises from synthesizing images, prior reports, and patient metadata. Benchmarks should stress visual grounding, temporal comparison, and contextual interpretation—not rely on text-only proxies.
    
    \item \textbf{Guard against saturation and overfitting:} Benchmarks should avoid becoming static targets. This requires continual refreshment, multiple blind test sets, and robust designs that resist memorization or shortcut exploitation.
\end{enumerate}

\subsection{Case Study: A Pilot Clinician-Annotated Benchmark for Report Generation}
\label{sec:report-benchmark}

As a step toward implementing our proposed design principles, we introduce a new benchmark for radiology report generation—one of the most clinically important and complex tasks in health AI.

Radiology report generation remains one of the most clinically valuable and technically demanding tasks in health AI. Yet, existing benchmarks—most notably MIMIC-CXR—rely on radiologist-written reports as gold-standard references, without acknowledging the ambiguity and variability inherent in clinical documentation. Inter-radiologist agreement for chest X-ray findings has been reported as low as 30\%~\cite{ref_disagreement}, and models are often evaluated against a single report with no structured ground truth.

Even with years of community effort, performance on MIMIC-CXR and similar datasets remains modest. Moreover, current benchmarks often provide limited support for understanding the cause of model failure—making it challenging to disentangle whether poor performance stems from model limitations or from shortcomings in benchmark design. Report generation is often treated as a monolithic task, lacking definition of what should be detected, described, or compared, and providing no path for attribution or error analysis.

To address this, we are developing a structured, clinician-annotated benchmark for radiology report generation. This pilot includes:
\begin{itemize}
    \item \textbf{Per-finding labels}: binary presence, severity, laterality, extent, and segmentation mask;
    \item \textbf{Temporal comparison}: improved/stable/worsened status vs. prior images;
    \item \textbf{Grounding}: matched phrases from the report for each finding;
    \item \textbf{Interpretation trace}: clinician reasoning actions (e.g., zooming, prior review) to support agentic modeling and evaluation.
\end{itemize}

Each case is labeled independently by three board-certified radiologists. We plan to release both a re-annotated version of the MIMIC-CXR test set and a new internal dataset drawn from previously unpublished clinical studies. This benchmark serves as a prototype for the principles proposed in this paper—clinically grounded, verifiable, and diagnostic. 

\textit{A detailed description of the dataset and annotation protocol will be presented in a forthcoming companion paper.}



==> arxiv2510/sections_v1/related.tex <==
% \section{Related Work: Benchmarking and Evaluation in Health AI}
% Benchmark-driven evaluation has played a central role in advancing health AI, providing standardized tasks and metrics to compare model capabilities. However, current benchmarks are highly fragmented—either focusing on textual reasoning divorced from visual context, or narrow vision-language tasks with limited clinical realism. In this section, we situate our work by reviewing the prevailing benchmark paradigms and highlighting where they fall short in evaluating models’ capacity for integrated, verifiable reasoning with medical images.

% \subsection{Text-Centric Benchmarks}
% A large body of benchmarks in health AI center on textual reasoning tasks derived from clinical exams or EHR-based datasets. Notable examples include MedQA-USMLE, PubMedQA, MedMCQA, and more recently, HealthBench and Med-Helm. These datasets have been instrumental in demonstrating that general-purpose large language models (LLMs) can match or exceed human performance on challenging medical questions.

% However, these benchmarks operate under the implicit assumption that all relevant clinical information—including visual findings—has already been converted into structured or unstructured text. They evaluate downstream inference while ignoring upstream visual uncertainty, diagnostic ambiguity, and perceptual errors that are common in real-world practice. As a result, these benchmarks decouple reasoning from its visual foundation, limiting their capacity to evaluate end-to-end clinical utility.

% \subsection{Vision-Language Benchmarks}
% Complementary efforts have explored the intersection of vision and language through tasks like visual question answering (VQA), image captioning, and radiology report generation. Datasets such as VQA-RAD, PathVQA, PMC-VQA, MIMIC-CXR, and IU-Xray provide multimodal benchmarks for evaluating the ability of models to interpret and describe medical images.

% These tasks offer critical insights into model perception and grounding, but often lack reasoning complexity. Many focus on single-turn queries or template-style generation, and do not require integration of prior knowledge, longitudinal comparison, or uncertainty handling. Vision-language models (VLMs) tuned on these datasets can excel by matching patterns rather than demonstrating true clinical reasoning.

% \subsection{Broad-Spectrum Benchmark Suites}
% Recent efforts like HealthBench and Med-Helm attempt to provide broader coverage by aggregating multiple tasks across different domains of health AI. These suites reflect an important trend toward comprehensive evaluation. However, they still rely exclusively on structured or textual inputs, implicitly assuming perfect visual interpretation upstream. Thus, while they capture diversity in reasoning styles, they remain blind to the perceptual challenges and propagation of errors originating from visual misinterpretation.

% \subsection{Agent-Based Reasoning and Emerging Capabilities}
% The next frontier in health AI evaluation lies in agentic reasoning—models that can plan, verify, and adapt across multi-step workflows. Frameworks like Microsoft’s Healthcare Agent Orchestrator, and the tool-use capabilities of GPT-4o and GPT-o3, point toward a shift in this direction. These models exhibit early-stage behaviors such as retrieving case-matched references, manipulating medical images (e.g., cropping, zooming), or routing to domain-specific tools.

% Yet, current benchmarks do not evaluate these capabilities systematically. Image manipulation, spatial reasoning, and cross-modality verification remain under-tested, despite their increasing importance in real-world clinical decision-making.

% \subsection{A Fragmented and Misaligned Landscape}
% Despite the diversity of existing benchmarks, a consistent pattern emerges: they are optimized for what is easy to measure, rather than what is essential to evaluate. Textual benchmarks ignore visual reasoning; vision-language benchmarks ignore context and clinical workflows; broad benchmark suites overlook perceptual errors entirely.

% In this work, we aim to bridge this gap. We reposition existing benchmarks along two critical dimensions—reasoning complexity and visual dependency—and introduce a rubric to make these dimensions explicit. This allows us to uncover latent failure modes in frontier models, identify what current benchmarks miss, and propose a more aligned path forward for evaluating health AI systems that reason with, not around, medical images.


\section{Related Work}

Recent advances in foundation models have propelled rapid progress across a wide range of health AI benchmarks. Yet, most of these benchmarks are optimized for isolated task success, rather than real-world readiness. In this section, we review the current landscape and highlight critical limitations that motivate our work.

\subsection{Health AI Benchmarks: Impressive Progress, Narrow Scope}


The past few years have seen a surge in benchmark development for health AI, reflecting growing interest in evaluating clinical reasoning, visual understanding, and multimodal capabilities. Text-based reasoning tasks such as MedQA, MedMCQA, and PubMedQA have become staples for evaluating large language models on biomedical knowledge recall. More recent efforts like HealthBench and Med-HELM broaden the scope by introducing open-ended prompts, clinician-authored rubrics, and multi-task taxonomies. On the visual side, benchmarks like VQA-RAD, PathVQA, and PMC-VQA test basic visual grounding, while MIMIC-CXR, RadGraph, and OpenI support radiology report generation. Generalist benchmarks like OmniMedVQA further expand modality and task diversity.

These benchmarks have enabled impressive progress. Modern LLMs now routinely surpass human scores on multiple-choice exams, and vision-language models (VLMs) achieve strong results in image captioning and visual question answering. This growth has helped drive community standards, unify task formats, and catalyze the development of increasingly capable foundation models for medicine.

Yet despite these advances, the scope of current benchmarks remains narrow. Many rely on simplified task formats—such as single-sentence factoid questions or multiple-choice prompts—that fail to capture the complexity of clinical decision-making. Others evaluate models on isolated modalities, with image inputs treated as auxiliary rather than central sources of evidence. Even multimodal benchmarks often stop short of testing true integrative reasoning across patient history, visual data, and temporal context. 

Critically, few benchmarks reflect the actual workflows of clinical care. Real-world decision-making is incremental, context-rich, and grounded in noisy and ambiguous data. It often requires reconciling multiple sources, navigating uncertainty, and revising prior conclusions. Yet these capabilities are rarely tested. Benchmarks also provide limited insight into model robustness, error recovery, or generalization across clinical domains.

This mismatch leads to an increasingly recognized failure mode: benchmark overfitting. Models optimized for specific leaderboards may appear state-of-the-art, yet falter on out-of-domain examples or clinically meaningful tasks. As a result, benchmark scores can give a false sense of readiness, while real clinical needs—such as trustworthy, verifiable, and context-aware AI systems—remain unmet.



\subsection{Benchmark Saturation and Spurious Progress}

Several recent papers have raised concerns about benchmark saturation, where new model iterations yield only marginal gains or outperform through shortcut learning, dataset leakage, or test set memorization \cite{placeholder_saturation1, placeholder_saturation2}. Models trained on overlapping datasets—sometimes unknowingly—have been shown to exploit stylistic or structural artifacts, inflating leaderboard rankings without meaningful generalization.

Moreover, benchmarks like ... have been partially included in model pretraining corpora or third-party instruction tuning datasets, further muddying the waters between fair evaluation and implicit leakage. Despite these issues, such benchmarks remain widely cited, with limited meta-evaluation on what they actually measure.

\subsection{Visual Reasoning and Multimodal Chain-of-Thought}

The capacity of models to reason with images—rather than simply classify them—has recently gained attention. Chain-of-thought prompting has been applied to medical VQA and radiology captioning, enabling models to generate stepwise inferences rather than short answers \cite{placeholder_cot1, placeholder_cot2}. Other approaches combine language models with perception modules and tool usage, as seen in recent work on agent-based clinical decision-making \cite{placeholder_agents1, placeholder_agents2}.

However, none of these approaches are benchmarked in a way that rewards verifiable visual reasoning. Models that attempt more complex chains of inference are not differentiated from those that guess based on prior distribution. There is no common rubric to assess when and how visual reasoning matters, or to penalize clinically dangerous hallucinations.

\subsection{Agentic Frameworks and Tool-Augmented Reasoning}

A growing body of work explores the use of LLMs as controllers in agentic frameworks, coordinating tools such as image segmentation, retrieval, or structured calculators for more verifiable and interactive clinical decision-making \cite{placeholder_agents1, placeholder_agents2}. In contrast to static end-to-end inference, these systems explicitly separate perception from reasoning and allow stepwise control over multimodal inputs.

Healthcare-specific frameworks have emerged to orchestrate domain-specialized models—e.g., for radiology, oncology, or genomics—under a central reasoning agent. These approaches promise stronger alignment with clinical workflows, but evaluation remains a challenge. Current benchmarks do not reward tool use, error correction, or visual traceability, making it difficult to compare agentic systems against monolithic baselines.


\subsection{Rethinking What We Measure in Health AI}

While there is growing recognition of the need for rigorous, clinically faithful evaluation in health AI \cite{placeholder_eval1, placeholder_eval2}, most current efforts remain benchmark-specific—expanding test sets, improving annotation, or refining metrics. Few attempt to ask the broader question: what should we be evaluating in the first place?

We argue that the field lacks a structured framework for assessing whether benchmarks reflect real-world complexity, visual grounding, or reasoning traceability. Without such guidance, model progress risks being misinterpreted—amplifying shallow shortcuts while missing deeper capabilities.

Rather than propose yet another benchmark, this paper takes a meta-evaluation perspective: we systematically reclassify existing benchmarks along clinically meaningful axes, analyze how current models succeed or fail under these conditions, and propose practical principles to guide benchmark design going forward.

In doing so, we aim to move the field beyond leaderboard chasing—toward evaluations that reflect the realities, risks, and reasoning required in actual clinical decision-making.





==> arxiv2510/sections_v1/result.tex <==
% \section{Frontier Model Performance Across Benchmarks}
% Despite achieving strong results on leaderboard metrics, frontier multimodal models reveal important failure patterns and emergent behaviors when evaluated across diverse health AI tasks. In this section, we analyze both quantitative outcomes and qualitative characteristics across benchmarks to surface current model limitations and unmeasured capabilities.

% \subsection{Models and Evaluation Protocol}

% We evaluate frontier multimodal models including GPT-4o, GPT-o3 (zero to high variants), GPT-o4-mini, Gemini-2.5-pro, and LLaVA-Med. For each, we test performance across the six benchmarks introduced in Section~\ref{sec:benchmark_repositioning}, which span increasing levels of visual and reasoning complexity.

% Each model is prompted with both direct and Chain-of-Thought (CoT) formats where applicable. For closed-ended tasks, we report accuracy; for open-ended generation, we use ROUGE or qualitative analysis. When models support real-time visual interaction (e.g., in GPT-o3 Web), we perform manual testing to explore emergent capabilities.

% We also compute a rubric-weighted composite score that incorporates benchmark complexity dimensions (visual, reasoning) as described in Section~\ref{sec:rubric_scoring}.

% \subsection{Quantitative Performance Across Tasks}

% Table~\ref{tab:all_results} summarizes benchmark-level accuracy across models. While models such as GPT-o3-high and Gemini-2.5-pro exceed 85\% accuracy on certain VQA tasks (e.g., OmniMedVQA), their performance drops sharply on open-ended or temporally grounded tasks like MIMIC-CXR and NEJM. Notably:

% \begin{itemize}
%     \item \textbf{GPT-o3-high} outperforms peers on complex cross-modality and case-based reasoning, but shows erratic performance on simpler VQA.
%     \item \textbf{Gemini-2.5-pro} achieves top accuracy on PMC-VQA but performs better in text-only mode than multimodal input for JAMA---a surprising result that suggests visual input can introduce noise or distract reasoning.
%     \item \textbf{Chain-of-Thought prompting} introduces verbosity without clear performance gain, and often reduces accuracy on short-form VQA (e.g., VQA-RAD).
% \end{itemize}


% \subsection{Emerging Model Behavior Patterns}
% Across tasks of varying complexity and modality alignment, several consistent behavior patterns emerge:

% \begin{itemize}
%     \item \textbf{Multimodal input generally improves performance, with notable exceptions.} Most models benefit from visual information on benchmarks requiring perceptual reasoning (e.g., NEJM). However, \textbf{Gemini-2.5-pro exhibits a 5-point performance drop on JAMA when provided with image inputs}, despite the task being largely text-resolvable. This anomaly, not observed in other models, suggests modality fusion challenges or over-reliance on irrelevant visual features.
    
%     \item \textbf{Increased reasoning capacity yields mixed returns.} While higher-tier GPT-o3 variants (e.g., \texttt{-high}) perform better on open-ended or cross-modality tasks, they underperform on simpler factoid-style benchmarks like VQA-RAD. This suggests potential overgeneration or instability in how internal reasoning chains are deployed across task types.
    
%     \item \textbf{Anatomical grounding and spatial reasoning remain brittle.} All evaluated models occasionally confuse laterality (e.g., left/right), mislabel anatomical regions, or hallucinate findings—especially in low-quality or ambiguous images. These errors often go undetected by current benchmarks, which lack the granularity to assess spatial correctness or uncertainty expression.

%     \item \textbf{to do}
% \end{itemize}


% \subsection{Emergent Visual Reasoning via Image Manipulation}
% We explore the emergent reasoning with image manipulation feature,   analyze 100 NEJM-style examples and find:

% \begin{itemize}
%     \item In 7x\% of cases, grounded manipulations (e.g., zooming into lung fields) correspond with correct diagnoses.
%     \item In 2x\%, manipulations are misaligned or superficial, reflecting hallucinated visual "moves" not grounded in actual image interpretation.
% \end{itemize}

% These results suggest the beginnings of \textit{agentic visual reasoning}, though health-specific tooling remains limited. Without DICOM viewers, region-of-interest operators, or structured anatomical primitives, current image manipulations remain shallow. Nonetheless, this signals a new modality for reasoning traceability.

% \subsection{Composite Score: Benchmarking Beyond Accuracy}

% To account for benchmark difficulty, we introduce a composite score:

% \[
% \text{Composite Score}_{m,t} = \frac{\text{Accuracy}_{m,t}}{1 + \text{Visual}_{t} + \text{Reasoning}_{t}}
% \]

% where $m$ indexes models and $t$ indexes tasks. Visual and reasoning scores are clinician-assigned rubric values (1–3). This score down-weights success on tasks solvable via text alone (e.g., JAMA) and up-weights high-dependency tasks (e.g., NEJM, MIMIC-CXR).

% When averaged across benchmarks, this yields a single composite metric per model—highlighting those most capable under realistic constraints. GPT-o3-high and Gemini-2.5-pro maintain top composite ranks, while LLaVA-Med, despite being vision-grounded, lags on both reasoning and generalization.

% \subsection{Emergent Behavior Patterns}

% Beyond accuracy, several behavioral patterns recur across tasks:

% \noindent \textbf{Visual inputs can degrade performance}. On JAMA (largely text-resolvable), Gemini-2.5-pro performs 5 points worse when images are included. This suggests susceptibility to irrelevant visual signals or failure to fuse modalities effectively.

% \noindent \textbf{Reasoning calibration is unstable}. GPT-o3-high performs best on complex tasks (NEJM, OmniMedVQA), yet underperforms on simpler tasks (VQA-RAD), revealing possible overfitting to multi-step patterns or unstable reasoning depth control.

% \noindent \textbf{Weak spatial and anatomical grounding}. All models exhibit left/right confusion, incorrect attribution of pathology locations, or hallucinations---especially in MIMIC-CXR where such errors would be clinically critical.


% \subsection{Emergent Visual Reasoning via Image Manipulation}

% Recent web-only releases of GPT-o3 and GPT-o4 series support real-time image manipulation (crop, rotate, zoom, sharpen), which can be used as reasoning steps. We manually evaluated 100 clinical cases and observed:

% \vspace{1em}
% \noindent \textbf{Key observations:}
% \begin{itemize}
%     \item \textbf{Models use image editing tools to generate more grounded and verifiable reasoning chains.} These manipulations are often accompanied by verbal justifications, producing a multi-modal chain-of-thought.
%     \item \textbf{No quantitative accuracy gains yet, but significantly more interpretable reasoning traces.} This suggests a shift from black-box outputs to transparent visual reasoning—an important step for clinical trust.
%     \item \textbf{These behaviors resemble agentic workflows}, where the model acts as a controller, dynamically coordinating with visual tools to iteratively refine its conclusions.
% \end{itemize}
% While currently unavailable via public APIs and limited by the absence of clinical image tools (e.g., DICOM viewer features, windowing), this capacity foreshadows a critical evolution: \textit{reasoning with images, not just about them}. We see this as a foundational component for next-generation, agent-based health AI systems.


% \subsection{Composite Scoring Reveals New Model Rankings}

% To go beyond task-specific accuracy, we compute a composite score for each model by weighting benchmark performance by the task’s reasoning and visual complexity scores (from Section 3). This re-ranks models in a clinically meaningful way. For example:

% \begin{itemize}
%     \item \textbf{GPT-o3-high} ranks higher than Gemini-2.5-pro despite lower raw accuracy on simpler benchmarks—reflecting its strength on complex reasoning tasks.
%     \item \textbf{Text-only models} score higher on low-complexity tasks, but fail to generalize to real-world, visual decision-making.
% \end{itemize}



\begin{table}[ht]
\centering
\caption{Performance on the VQA-RAD benchmark, a short-form single-modality visual question answering dataset focused on radiographic reasoning.}
\label{tab:vqa_rad}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o         & 100 & 63\% \\
GPT-4o + CoT   & 100 & 60\% \\
GPT-o3         & 100 & 66\% \\
GPT-o3 + CoT   & 100 & 63\% \\
GPT-o4-mini    & 100 & 59\% \\
GPT-o4-mini + CoT   & 100 & 61\% \\
Gemini-2.5-pro  & 100 & 67\% \\
Gemini-2.5-pro + CoT   & 100 & 64\% \\
GPT-5         & 100 & 66\% \\
GPT-5 + CoT   & 100 & 65\% \\
\midrule
GPT-4o         & 451 & 60.98\% \\
o3         & 451 & 65.63\% \\
o4-mini    & 451 & 64.08\% \\
Gemini-2.5-pro & 451 & 66.30\% \\
Deepseek       & 451 & 45.68\% \\
Llava-med-1.5  & 451 & 44.35\%\\
GPT-5         & 451 & \textbf{67.85}\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Results on PMC-VQA, a cross-modality benchmark containing open-ended questions grounded in biomedical literature and image context.}
\label{tab:pmc_vqa}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o             & 486 & 50.21\% \\
o3-zero        & 486 & 60.08\% \\
% GPT-o3-low         & 100 & 52.63\% \\
% GPT-o3-medium      & 100 & 57.89\% \\
% GPT-o3-high        & 100 & 57.89\% \\
o4-mini-zero   & 486 & 59.47\% \\
Gemini-2.5-pro     & 486 & 58.44\% \\
Deepseek           & 486 & 40.95\% \\
Llava-med-1.5      & 486 & 6.17\%\\
Voting(x5)      & 486 &  62.35\%\\
Voting(x4)      & 486 &  62.76\%\\
Voting(x3)      & 486 &  60.91\%\\
GPT-5           & 486 &  58.85\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Performance on OmniMedVQA, a comprehensive benchmark spanning 73 medical datasets and 12 imaging modalities, designed to evaluate generalist medical visual reasoning.}
\label{tab:omnimedvqa}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Total Samples} & \textbf{Accuracy} \\
\midrule
GPT-4o             & 517 & 73.31\% \\
GPT-o3             & 517 & 85.49\% \\
GPT-o3-low         & 517 & 84.91\% \\
GPT-o3-medium      & 517 & 84.99\% \\
GPT-o3-high        & 517 & 86.65\% \\
GPT-o4-mini        & 517 & 81.43\% \\
Gemini-2.5-pro     & 517 & 85.69\% \\
Deepseek           & 517 & 54.01\% \\
Llava-med-1.5      & 517 & 68.66\% \\
Voting(x5)             & 517 & 86.46\% \\
Voting(x4)             & 517 & 86.46\% \\
Voting(x3)             & 517 & 87.62\% \\
GPT-5             & 517 & \textbf{87.43}\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Accuracy on challenging real-world case questions from JAMA Clinical Challenge and NEJM Case Reports. These benchmarks assess multi-step reasoning and domain-specific clinical understanding.}
\label{tab:clinical_cases}
\begin{tabular}{lcc}
\toprule
\textbf{Benchmark} & \textbf{Model} & \textbf{Accuracy} \\
\midrule
JAMA   & GPT-o3-zero      & 84.75\% \\
JAMA   & Gemini-2.5-pro   & 84.36\% \\
NEJM   & GPT-o3-zero      & 80.89\% \\
NEJM   & Gemini-2.5-pro   & 80.89\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Model accuracy on JAMA clinical case challenge.}  
JAMA cases are predominantly solvable via text alone.  
Text-only models perform competitively, and in some cases (e.g., Gemini-2.5-pro), outperform their multimodal counterparts.   
Filtered inputs reflect examples where image access was blocked by safety mechanisms.}

\begin{tabular}{llcc}
\toprule
\textbf{Model} & \textbf{Input Type} & \textbf{\# Examples} & \textbf{Accuracy (\%)} \\
\midrule
o3        & Image + Text (filtered) & 1141 & 84.75 \\
o4-mini   & Image + Text (filtered) & 1156 & 80.36 \\
o4-mini   & Image + Text (filtered) & 1141 & 80.46 \\
GPT-4o             & Image + Text            & 1314 & 69.10 \\
GPT-4o             & Image + Text (filtered) & 1141 & 69.94 \\
Gemini-2.5-pro     & Image + Text            & 1314 & 84.36 \\
Gemini-2.5-pro     & Image + Text (filtered) & 1141 & \textbf{84.84} \\
Deepseek           & Image + Text            & 1314 & 38.96 \\
Deepseek           & Image + Text (filtered) & 1141 & 38.21 \\
LLaVA-Med          & Image + Text            & 1314 & 22.54 \\
LLaVA-Med          & Image + Text (filtered) & 1141 & 22.74 \\
Voting(x5)         & Image + Text            & 1141 & 84.66 \\
Voting(x4)         & Image + Text            & 1141 & 85.54 \\
Voting(x3)         & Image + Text            & 1141 & 86.06 \\
GPT-5              & Image + Text            & 1314 & \textbf{86.83} \\
GPT-5              & Image + Text (filtered) & 1141 & \textbf{86.59} \\

\addlinespace
o3             & Text Only               & 1314 & 82.42 \\
o3             & Text Only (filtered)    & 1141 & \textbf{82.65} \\
o4-mini        & Text Only               & 1314 & 77.70 \\
o4-mini        & Text Only (filtered)    & 1141 & 78.44 \\
Gemini-2.5-pro     & Text Only               & 1314 & 74.58 \\
Gemini-2.5-pro     & Text Only (filtered)    & 1141 & 74.93 \\
GPT-4o             & Text Only               & 1314 & 68.34 \\
GPT-4o             & Text Only (filtered)    & 1141 & 68.89 \\
Deepseek           & Text Only               & 1314 & 33.33 \\
Deepseek           & Text Only (filtered)    & 1141 & 32.60\\
GPT-5              & Text Only               & 1314 & \textbf{82.57} \\
GPT-5              & Text Only (filtered)    & 1141 & \textbf{82.91} \\

\bottomrule
\end{tabular}
\label{tab:jama_cases}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Model accuracy on NEJM clinical case challenge.} These tasks require visual reasoning and context integration. Multimodal models clearly outperform text-only models.}
\begin{tabular}{llcc}
\toprule
\textbf{Model} & \textbf{Input Type} & \textbf{\# Examples} & \textbf{Accuracy (\%)} \\
\midrule
Gemini-2.5-pro     & Image + Text           & 947 & 80.89 \\
Gemini-2.5-pro(06) & Image + Text           & 947 & 83.14 \\
Gemini-2.5-pro     & Image + Text (filtered) & 743 & 79.95 \\
Gemini-2.5-pro(06)    & Image + Text (filtered) & 743 & 83.74 \\
o3-zero        & Image + Text (filtered) & 743 & 80.89 \\
o4-mini-zero   & Image + Text (filtered) & 743 & 75.91 \\
GPT-4o             & Image + Text           & 947 & 66.53 \\
GPT-4o             & Image + Text (filtered) & 743 & 66.90 \\
Deepseek           & Image + Text & 947 & 33.16 \\
Llava-med          & Image + Text              & 947 & 29.04 \\
voting (x5)        & Image + Text              & 743 &  80.48\\
voting (x4)        & Image + Text              & 743 &  80.62\\
voting (x3)        & Image + Text              & 743 &  81.83\\
GPT-5           & Image + Text             & 947 & 81.10 \\
GPT-5           & Image + Text (filtered)      & 743 & 80.89 \\



\addlinespace
o3             & Text Only              & 947 & \textbf{67.69} \\
o3             & Text Only  (filtered)  & 743 & \textbf{67.03} \\
o4-mini        & Text Only              & 947 & 66.42 \\
o4-mini        & Text Only  (filtered)  & 743 & 66.49 \\
Gemini-2.5-pro(06) & Text Only              & 947 & 67.16 \\
Gemini-2.5-pro(06) & Text Only  (filtered)  & 743 & 67.56\\
Gemini-2.5-pro     & Text Only              & 947 & 65.01 \\
Gemini-2.5-pro     & Text Only  (filtered)  & 743 & 65.01\\
GPT-4o             & Text Only              & 947 & 37.38 \\
GPT-4o             & Text Only              & 743 & 37.28 \\
Deepseek           & Text Only              & 947 & 25.34 \\
Deepseek           & Text Only              & 743 & 25.30 \\
GPT-5           & Text Only              & 947 & \textbf{67.79} \\
GPT-5           & Text Only              & 743 & \textbf{67.56} \\

\\
Gemini-2.5-pro     & Image + Text           & 118 & 82.22 \\
Gemini-2.5-pro + cot & Image + Text         & 118 & 81.36 \\
o3-zero        & Image + Text           & 118 & 80.51 \\
o3-zero + cot  & Image + Text           & 118 & 79.66 \\
o4-mini-zero   & Image + Text           & 118 & 74.58 \\
o4-mini-zero + cot  & Image + Text      & 118 & 79.66 \\
GPT-4o             & Image + Text           & 118 & 66.95 \\
GPT-4o + cot       & Image + Text           & 118 & 65.25 \\
GPT-5             & Image + Text           & 118 & 81.36 \\
GPT-5 + cot       & Image + Text           & 118 & 79.66 \\

\bottomrule
\end{tabular}
\label{tab:nejm_cases}
\end{table}


% \begin{table}[ht]
% \centering
% \caption{Summary of benchmark characteristics and best performance. Visual dependency and reasoning complexity are clinician-verified rubric scores (1=Low, 3=High).}
% \label{tab:benchmark_summary}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Benchmark} & \textbf{Task Type} & \textbf{Visual Dep.} & \textbf{Reasoning Comp.} & \textbf{Best Accuracy (Model)} \\
% \midrule
% VQA-RAD      & Image-only VQA       & 2 & 1 & 64.97\% (GPT-o3) \\
% PMC-VQA      & Cross-modal VQA      & 2 & 2 & 60\% (GPT-o3-zero) \\
% OmniMedVQA   & Cross-modal VQA      & 3 & 2 & 85.8\% (GPT-o3-high) \\
% JAMA Cases   & Clinical case VQA  & 1 & 3 & 86.6\% (GPT-o3-zero) \\
% NEJM Cases   & Clinical case VQA    & 3 & 3 & 80.9\% (GPT-o3-zero, Gemini) \\
% MIMIC-CXR   & Report Gen.    & 3 & 2 & xx \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{table}[htbp]
\centering
\caption{Report evaluation results across different models.}
\begin{tabular}{lccccc}
\hline
Model & 1/RadCliQ-v1 & BLEU Score & BERT Score & Semantic Score & RadGraph F1\\
\hline
GPT-4V & 0.568 & 0.075 & 0.214 & 0.337 & 0.138\\
GPT-4o & 0.670 & 0.098 & 0.289 & 0.291 & 0.153\\
GPT-5 & 0.628 & 0.090  & 0.251 & 0.271 & 0.140 \\
o3 & 0.596 & 0.084 & 0.210 & 0.260 & 0.135 \\
o3 (high) & 0.602 & 0.085 & 0.217 & 0.264 & 0.136 \\
o4-mini & 0.626 & 0.091 & 0.233 & 0.284 & 0.148 \\
Gemini-2.5-pro & 0.648 & 0.100 & 0.257 & 0.307 & 0.143 \\
Deepseek & 0.496 & 0.047 & 0.094 & 0.198  & 0.066 \\
MAIRA & 1.008 & 0.205 & 0.436 & 0.462 & 0.187\\
MedVERSA & 1.008 & 0.210 & 0.431 & 0.498 & 0.202\\
\hline
\end{tabular}
\label{tab:report_evaluation_results}
\end{table}


\begin{table}[ht]
\centering
\caption{Performance of different models under various prompt modifications on NEJM dataset. Accuracy is reported separately for text-only and visual-answerable settings.}
\small
\begin{tabular}{lllrr}
\hline
\textbf{Model} & \textbf{Version} & \textbf{Modified} & \textbf{Text Acc. (\%)} & \textbf{Visual Acc. (\%)} \\
\hline
GPT-4o    & v9  & no                  & 3.43 & 46.29 \\
GPT-4o    & v8  & 0-replace, reord    & 0.57 & 46.85 \\
GPT-4o    & v7  & 1-replace, reord    & 1.71 & 50.28 \\
GPT-4o    & v6  & 2-replace, reord    & 2.28 & 54.28 \\
GPT-4o    & v5  & 3-replace, reord    & 0.37 & 65.14 \\
GPT-4o    & v4  & 4-replace, reord    & 2.28 & 84.00 \\

\\

o4-mini    & v9  & no                  & 33.71 & 58.86 \\
o4-mini    & v8  & 0-replace, reord    & 33.71 & 55.43 \\
o4-mini    & v7  & 1-replace, reord    & 36.57 & 62.37 \\
o4-mini    & v6  & 2-replace, reord    & 32.57 & 68.57 \\
o4-mini    & v5  & 3-replace, reord    & 24.57 & 73.72 \\
o4-mini    & v4  & 4-replace, reord    & 17.14 & 85.14 \\

\\
Gemini-2.5-pro  & v9  & no                  & 37.14 & 67.42 \\
Gemini-2.5-pro  & v8  & 0-replace, reord    & 33.14 & 70.28 \\
Gemini-2.5-pro  & v7  & 1-replace, reord    & 38.86 & 72.00 \\
Gemini-2.5-pro  & v6  & 2-replace, reord    & 35.42 & 73.71 \\
Gemini-2.5-pro  & v5  & 3-replace, reord    & 26.85 & 82.29 \\
Gemini-2.5-pro  & v4  & 4-replace, reord    & 17.14 & 92.57 \\

\\
o3         & v9  & no                  & 37.71 & 61.71 \\
o3         & v8  & 0-replace, reord    & 31.42 & 64.00 \\
o3         & v7  & 1-replace, reord    & 29.71 & 68.57 \\
o3         & v6  & 2-replace, reord    & 27.42 & 70.86 \\
o3         & v5  & 3-replace, reord    & 21.14 & 80.57 \\
o3         & v4  & 4-replace, reord    & 20.00 & 89.14 \\


\\
GPT-5         & v9  & no                  & 37.71 & 66.28 \\
GPT-5         & v8  & 0-replace, reord    & 32.00 & 70.85 \\
GPT-5         & v7  & 1-replace, reord    & 33.14 & 69.71 \\
GPT-5         & v6  & 2-replace, reord    & 29.24 & 73.71 \\
GPT-5         & v5  & 3-replace, reord    & 24.27 & 86.29 \\
GPT-5         & v4  & 4-replace, reord    & 20.00 & 90.86 \\
\hline
\end{tabular}
\label{tab:model_nejm_performance}
\end{table}


\begin{table}[ht]
\centering
\caption{Performance of different models on the NEJM subset under prompt modifications that randomly replace one non-ground-truth option with \texttt{"unknown"}. 
Accuracy is reported separately for text-only and visual-answerable settings. 
All models show improved accuracy after this modification, suggesting that the gain may stem from pattern recognition or shallow matching rather than true reasoning. 
Given that no images are provided in the original questions, a reasonable answer to the text-only modified prompt should be \texttt{"unknown"}.
}
\small
\begin{tabular}{lllrr}
\hline
\textbf{Model} & \textbf{Version} & \textbf{Modified} & \textbf{Text Acc. (\%)} & \textbf{Visual Acc. (\%)} \\
\hline
GPT-4o    & v9  & no                    & 3.43 & 46.29 \\
GPT-4o    & v11 & 1-replace, “unknown”  & 4.57 & 53.71 \\
\\
o4-mini    & v9  & no                  & 33.71 & 58.86 \\
o4-mini    & v11 & 1-replace, “unknown”  & 42.28 & 61.14 \\
\\
Gemini-2.5-pro  & v9  & no                  & 37.14 & 67.42 \\
Gemini-2.5-pro  & v11 & 1-replace, “unknown”  & 45.71 & 69.71 \\
\\
o3         & v9  & no                  & 37.71 & 61.71 \\
o3         & v11 & 1-replace, “unknown”  & 34.28 & 67.43 \\
\\
GPT-5      & v9  & no                    & 37.71 & 66.28 \\
GPT-5      & v11 & 1-replace, “unknown”  & 42.86 & 71.73 \\
\hline
\end{tabular}

\label{tab:model_nejm_performance_unknown}
\end{table}


\begin{table}[ht]
\centering
\caption{Original vs.\ image-augmented question accuracies. Image-augmented results are obtained by evaluating 40 questions across three trials (120 total VQA evaluations). The baseline repeats the original questions across multiple trials to match the same evaluation budget.}

\small
\begin{tabular}{lccc}
\hline
{Model} & {Original (\%)} & {Image-aug (\%)} & {$\Delta$ Acc.} \\
% Model   & Original Acc. (\%) & Image-aug Acc. (\%) & {$\Delta$ (pp)}\\
\hline
Gemini-pro  & 80.83 & 47.50 & -33.33 \\
GPT-5   & 83.33 & 51.67 & -31.66\\
o3      & 76.67 & 52.50 & -24.17\\
o4-mini & 71.67 & 37.50 & -34.17\\
GPT-4o  & 36.67 & 41.67 & +5.00\\
\hline
\end{tabular}

\label{tab:model_nejm_image_aug}
\end{table}


\begin{table}[ht]
\centering
\caption{Accuracy (\%) of different models across categories on JAMA dataset.}
\begin{tabular}{l|c|cccc}
\toprule
\textbf{Model} & \textbf{Type} & \textbf{Operation} & \textbf{Diagnosis}  \\
\midrule

Gemini-2.0-flash & visual  & 30.15 & 45.82  \\
Gemini-2.5-pro   & visual  & 80.72 & \textbf{89.35}  \\
GPT-4o           & visual  & 66.72 & 73.57  \\
o3           & visual  & \textbf{80.89} & 88.97  \\
o4-mini          & visual  & 75.95 & 85.55  \\
GPT-5            & visual  & \textbf{84.02} &  \textbf{89.35} \\
\\
Gemini-2.0-flash & text & 32.29 & 38.21  \\
Gemini-2.5-pro   & text & 69.85 & 80.80  \\
GPT-4o           & text & 65.40 & 72.81  \\
o3           & text & \textbf{78.75} & \textbf{87.07}  \\
o4-mini          & text & 76.61 & 80.61  \\
GPT-5            & text  & \textbf{78.91} & \textbf{87.45}  \\
\bottomrule
\end{tabular}
\label{tab:jama_model_acc}
\end{table}

==> arxiv2510/sections_v1/result_2.tex <==
\section{Evaluating Multimodal Models on Clinical Tasks}

Despite impressive performance on leaderboards, frontier multimodal models often fail in clinically critical ways. In this section, we evaluate leading LMMs across a suite of health benchmarks that span short-form visual question answering (VQA), biomedical literature-grounded inference, case-based diagnostic reasoning, and radiology report generation. Our analysis highlights gaps between benchmark performance and real-world reliability—revealing patterns of degradation, spurious modality effects, and limitations in anatomical grounding.

\subsection{Models and Evaluation Protocol}

We evaluate state-of-the-art LMMs, including GPT-4o, GPT-o3 (multiple variants), GPT-o4-mini, Gemini 2.5 Pro, DeepSeek-VL, and LLaVA-Med. Each model is tested across six benchmarks that vary in visual complexity and reasoning demands: VQA-RAD, PMC-VQA, OmniMedVQA, JAMA Clinical Challenge, NEJM Case Reports, and MIMIC-CXR report generation.

Benchmarks are grouped by input-output style (e.g., closed-form classification vs. open-ended generation). Where appropriate, we evaluate both direct prompting and Chain-of-Thought (CoT) prompting. Metrics include accuracy for classification tasks, and ROUGE, BLEU, and clinically validated metrics such as RadGraph F1 for report generation.

\vspace{0.5em}
\noindent Table~\ref{tab:benchmark_summary} summarizes benchmark characteristics and top-performing models.

\begin{table}[ht]
\centering
\caption{\textbf{Overview of clinical benchmarks and best-performing models.} Benchmarks vary by task format and required visual reasoning. Scores reflect raw accuracy or inverse error (RadCliQ$\downarrow$) as applicable.}
\label{tab:benchmark_summary}
\begin{tabular}{lccc}
\toprule
\textbf{Benchmark} & \textbf{Task Type} & \textbf{Best Score} & \textbf{Best Model} \\
\midrule
VQA-RAD       & Radiographic VQA        & 66.3\% & Gemini-2.5-pro \\
PMC-VQA       & Biomedical literature VQA & 60.1\% & GPT-o3-zero \\
OmniMedVQA    & Generalist medical VQA  & 87.6\% & GPT-o3-high (Voting) \\
JAMA Cases    & Diagnostic reasoning (text-heavy) & 86.1\% & GPT-o3-zero (Voting) \\
NEJM Cases    & Diagnostic reasoning (image-grounded) & 83.7\% & Gemini-2.5-pro \\
MIMIC-CXR     & Report generation       & 1.008 (RadCliQ$\downarrow$) & MedVERSA \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Quantitative Performance Across Tasks}

Across benchmarks, LMMs achieve high scores on short-form tasks but struggle with complex, temporally grounded, or image-intensive cases.

\begin{itemize}
    \item \textbf{OmniMedVQA and JAMA} yield the highest raw scores, suggesting models excel in short-form or predominantly text-resolvable settings (Tables~\ref{tab:omnimedvqa} and~\ref{tab:jama_cases}).
    \item \textbf{NEJM and MIMIC-CXR} reveal deeper failure points: subtle anatomical mislocalizations, overgeneralized findings, or incorrect diagnostic attribution (Tables~\ref{tab:nejm_cases},~\ref{tab:report_evaluation_results}).
    \item \textbf{Image modality fusion can degrade performance}. In JAMA, Gemini-2.5-pro achieves higher accuracy with text-only input than with image+text, indicating sensitivity to irrelevant visual cues.
\end{itemize}

\subsection{Emergent Behavior Patterns}

Beyond raw accuracy, evaluation surfaces consistent patterns of behavior across models:

\vspace{0.5em}
\noindent\textbf{Visual input does not always help}. Although visual grounding is critical in real practice, models sometimes perform better without images. On JAMA, text-only inputs improve accuracy by up to 5 points in Gemini-2.5-pro (Table~\ref{tab:jama_cases}).

\vspace{0.5em}
\noindent\textbf{Reasoning robustness is uneven}. GPT-o3-high achieves top performance on complex benchmarks like NEJM and OmniMedVQA, but underperforms on simpler datasets like VQA-RAD—suggesting instability in reasoning depth calibration.

\vspace{0.5em}
\noindent\textbf{Spatial grounding remains brittle}. Left/right confusion, anatomical hallucinations, and low-quality image sensitivity persist, particularly in MIMIC-CXR. These errors are rarely caught by benchmark metrics, but could carry clinical risk in practice.

\subsection{Visual Reasoning via Image Manipulation}

A new emergent capability in web-based versions of GPT-o3 and GPT-o4 is real-time image manipulation (zoom, rotate, sharpen), which can function as steps in visual reasoning. We evaluated 100 clinical cases where this feature was available and observed:

\begin{itemize}
    \item Models often use image operations to generate more traceable, multimodal reasoning chains.
    \item Although quantitative gains are unclear, interpretability improves—suggesting potential for future interactive systems.
    \item These behaviors resemble early forms of agentic reasoning, where models orchestrate visual exploration to guide conclusions.
\end{itemize}

While these capabilities are not yet available in APIs and lack clinical tooling (e.g., DICOM viewers), they point toward an important frontier: reasoning \textit{with} medical images, not just \textit{about} them.

\subsection{Model Rankings Depend on Benchmark Context}

Model rankings vary widely depending on the benchmark. GPT-o3-high ranks highest on clinically grounded tasks like NEJM, while Gemini-2.5-pro leads on text-dominant challenges like JAMA and PMC-VQA. However, these raw scores may misrepresent model robustness in more realistic settings—a question we revisit in Section~\ref{sec:rubric} through rubric-based composite evaluation.

\begin{table}[ht]
\centering
\caption{\textbf{Performance on visual question answering benchmarks.} Tasks differ in complexity, with OmniMedVQA covering a broad set of modalities.}
\label{tab:vqa_aggregate}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{VQA-RAD} & \textbf{PMC-VQA} & \textbf{OmniMedVQA} \\
\midrule
GPT-4o             & 60.98\% & 50.21\% & 73.31\% \\
GPT-o3             & 65.63\% & 60.08\% & 85.49\% \\
GPT-o3-high        & --      & --      & \textbf{86.65\%} \\
Gemini-2.5-pro     & \textbf{66.30\%} & 58.44\% & 85.69\% \\
DeepSeek           & 45.68\% & 40.95\% & 54.01\% \\
LLaVA-Med          & 44.35\% & 6.17\%  & 68.66\% \\
Voting (x3)        & --      & 60.91\% & \textbf{87.62\%} \\
\bottomrule
\end{tabular}
\end{table}


==> arxiv2510/sections_v2/appendex.tex <==
\clearpage
\section{Robustness Score Computation}
\label{app:robustness}
We quantify overall stability using a \textbf{Robustness Score}.  
For each stress test $T_i$ ($i=1 \ldots 5$) and model $m$, we compute a fragility value $f_i(m) \in [0,1]$.  
Robustness for that test is defined as
\[
r_i(m) = 1 - f_i(m),
\]
and the mean robustness score is given by the unweighted average
\[
R(m) = \frac{1}{5} \sum_{i=1}^{5} r_i(m).
\]

The fragility components $f_i(m)$ are defined as follows:

\paragraph{T1: Modality Sensitivity.}  
Weighted performance drop when image input is removed on JAMA and NEJM:
\[
f_1(m) = \frac{n_{\text{JAMA}} \cdot \max\!\big(0, \, \text{Acc}^{\text{img}}_{\text{JAMA},m} - \text{Acc}^{\text{text}}_{\text{JAMA},m}\big) 
        + n_{\text{NEJM}} \cdot \max\!\big(0, \, \text{Acc}^{\text{img}}_{\text{NEJM},m} - \text{Acc}^{\text{text}}_{\text{NEJM},m}\big)}
       {100 \cdot (n_{\text{JAMA}} + n_{\text{NEJM}})}.
\]

\paragraph{T2: Modality Necessity.}  
Excess accuracy above chance (20\%) when images are withheld on visually required items:
\[
f_2(m) = \frac{\max\!\big(0, \, \text{Acc}^{\text{text}}_{\text{vis-req},m} - 20\big)}{80}.
\]

\paragraph{T3: Format Perturbation.}  
Accuracy drop in text-only condition after reordering answer options:
\[
f_3(m) = \frac{\max\!\big(0, \, \text{Acc}^{\text{text-orig}}_m - \text{Acc}^{\text{text-reord}}_m\big)}{100}.
\]

\paragraph{T4: Distractor Replacement.}  
Composite fragility capturing text-mode degradation, image-mode gain under distractor removal, and gains when inserting ``Unknown'' distractors. Weights of 0.5, 0.3, and 0.2 were applied, respectively:
\[
\begin{aligned}
f_4(m) &= 0.5 \cdot \frac{\max\!\big(0, \, \text{Acc}^{\text{text-base}}_m - \text{Acc}^{\text{text-4R}}_m\big)}{100} \\
       &+ 0.3 \cdot \frac{\max\!\big(0, \, \text{Acc}^{\text{img-4R}}_m - \text{Acc}^{\text{img-base}}_m\big)}{100} \\
       &+ 0.2 \cdot \frac{\max\!\big(0, \, \text{Acc}^{\text{text-UNK}}_m - \text{Acc}^{\text{text-base-UNK}}_m\big)}{100}.
\end{aligned}
\]

\paragraph{T5: Visual Substitution.}  
Performance drops when the original image is replaced with a distractor-aligned substitute:
\[
f_5(m) = \frac{\max\!\big(0, \, \text{Acc}^{\text{orig}}_m - \text{Acc}^{\text{subst}}_m\big)}{100}.
\]




\vspace{5mm}
\section{More stress test results}
\label{app:stress test}

In this appendix, we present several case studies from the stress-testing experiments. Each figure illustrates a group of stress tests applied to a single question, highlighting model behaviors under controlled perturbations.

Figures~\ref{fig:no_image_example_1}-\ref{fig:no_image_example_3} show representative examples of \textbf{stress test 2 and 3} (Section~\ref{sec:stress-tests}). These cases demonstrate how models often rely on textual shortcuts: when visual information is removed, most models still produce seemingly correct answers by exploiting superficial textual cues rather than genuine multimodal reasoning. In contrast, GPT-4o is the only model that consistently abstains or selects “Unknown” in the absence of the image.

Figures ~\ref{fig:image_replaced_example_1}-\ref{fig:image_replaced_example_3} illustrate \textbf{stress test 5}, which probe visual comprehension under visual substitution. A model with true visual understanding should revise its prediction to align with the substituted image. Instead, performance collapses across all models, revealing that models' reliance on shortcut strategies and their limited ability to incorporate visual evidence, whereas accurate performance would require aligning predictions with the substituted image. Once shortcut strategies are disrupted, their true comprehension is far weaker than the benchmark scores suggest.

% add notes
\vspace{0.5em}
\noindent {\footnotesize\textit{Note:} Based on the modality and anatomical location of the original problem image, we retrieved candidate distractor images using Google Image Search~\cite{google_search}. These candidates were visually similar to the original but depicted different conditions. To ensure validity, each image was manually reviewed to verify consistency between the visual content and the associated disease label.}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/NEJM_no_image_example_1}
 
    \caption{\textbf{Illustration of model behavior under Stress Tests 2 and 3: Case 1}. We apply three modifications to the original image-based multiple-choice question (ground truth: Dermatomyositis): (i) remove the image, (ii) shuffle the answer options, and (iii) replace one option with “Unknown.” When the image is absent, the appropriate behavior is to abstain (or to select “Unknown” if available). However, most models still provide a diagnosis—often repeating Dermatomyositis even after the options are shuffled—whereas GPT-4o is the only model that consistently refuses to answer without the image.}
    \label{fig:no_image_example_1}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/NEJM_no_image_example_2}
    \caption{\textbf{Illustration of model behavior under Stress Tests 2 and 3: Case 2}. We apply three modifications to the original image-based multiple-choice question (ground truth: Chiari I malformation): (i) remove the image, (ii) shuffle the answer options, and (iii) replace one option with “Unknown.” When the image is absent, the expected behavior is to abstain (or to select “Unknown” if available). Nevertheless, most models continue to provide a diagnosis—often repeating the original ground truth—whereas GPT-4o is the only model that consistently either abstains or selects “Unknown” in the absence of the image.}
    \label{fig:no_image_example_2}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/NEJM_no_image_example_3}
    \caption{\textbf{Illustration of model behavior under Stress Tests 2 and 3: Case 3}. We apply three modifications to the original image-based multiple-choice question (ground truth: Pneumatosis cystoides coli): (i) remove the image, (ii) shuffle the answer options, and (iii) replace one option with “Unknown.” When the image is absent, the expected behavior is to abstain (or to select “Unknown” if available). Nevertheless, most models continue to provide a diagnosis—often repeating the original ground truth—whereas GPT-4o is the only model that consistently refuses to answer without the image.}
    \label{fig:no_image_example_3}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/stress_image_replaced_example_1}
    \caption{\textbf{Illustration of model behavior under Stress Test 5 (Visual Substitution): Case 4}. The original question image is replaced with medical images corresponding to distractor options (Endocarditis, Lichen planus, Porphyria). }
    \label{fig:image_replaced_example_1}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/stress_image_replaced_example_2}
    \caption{\textbf{Illustration of model behavior under Stress Test 5 (Visual Substitution): Case 5}. The original question image is replaced with medical images corresponding to distractor options (Cerebral aneurysm, Neurofibromatosis, Paget disease).}
    \label{fig:image_replaced_example_2}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/stress_image_replaced_example_3}
    \caption{\textbf{Illustration of model behavior under Stress Test 5 (Visual Substitution): Case 6}. The original question image is replaced with medical images corresponding to distractor options (Empyema, Lymphangioleiomyomatosis, Pericardial effusion).}
    \label{fig:image_replaced_example_3}
\end{figure}

\vspace{5mm}
\section{More reasoning failure results}
\label{app:reasoning}
As discussed in Section~\ref{sec:stress-tests}, we identify several key patterns of reasoning failure: incorrect logic despite correct answers, reinforced visual misunderstandings, and uninformative reasoning steps. In this appendix, we present additional illustrative cases of these failure modes in Figures~\ref{fig:error_reason_heuristic}–\ref{fig:error_reason_misgrounded}. These cases further demonstrate how such reasoning errors manifest across different tasks and inputs.



\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/error_reason_heuristic}
    \caption{\textbf{Reasoning failure pattern: confident but false heuristic.} Two representative cases in which the model relies on a plausible yet incorrect prior rather than performing accurate visual interpretation, resulting in systematic errors.}
    \label{fig:error_reason_heuristic}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/error_reason_hullucinated}
    \caption{\textbf{Reasoning failure pattern: correct answer but hallucinated perception.} Two representative cases where the model produces the correct output despite lacking substantive utilization of image content, indicating dependence on non-visual shortcuts.  }
    \label{fig:error_reason_hullucinated}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]
    {figures/error_reason_misgrounded}
    \caption{\textbf{Reasoning failure pattern: visual reasoning with faulty grounding.} Two examples where the model performs step‑by‑step image analysis but bases its reasoning on inaccurate or imagined features, producing confident yet incorrect conclusions.  }
    \label{fig:error_reason_misgrounded}
\end{figure}

\vspace{5mm}
\section{Evaluation on report generation task}
\label{app:report_genenration}
 
Extented Data Table~\ref{tab:report_evaluation} summarizes the report generation performance on the MIMIC-CXR test set for both general-purpose LMMs and specialized medical models (e.g., MAIRA-2~\cite{bannur2024maira2}, MedVERSA~\cite{zhou2024medversa}). 
Evaluation is conducted with five complementary metrics: (1) $1/\text{RadCliQ-v1}$, where higher values indicate better clinical correctness per the RadCliQ composite metric~\cite{roberts2021radcliq}; (2) BLEU Score, measuring n-gram overlap with reference reports~\cite{papineni2002bleu}; (3) BERT Score, assessing semantic similarity via contextual embeddings~\cite{zhang2020bertscore}; (4) Semantic Score, capturing higher-level alignment of generated and reference report content~\cite{irvin2019chexpert}; and (5) RadGraph F1, evaluating extraction accuracy of clinical entities and relations from generated reports~\cite{jain2021radgraph}.   
Across all metrics, MedVERSA achieves the highest performance, particularly in semantic alignment and clinical information extraction. Its advantage stems from domain-specific training on paired image–text data, which enables mastery of radiological terminology, fine-grained visual patterns, and clinical reasoning. In contrast, general-purpose LMMs lack such specialization, limiting their ability to capture subtle radiographic findings.

Among the general-purpose models, GPT-4o and Gemini-2.5 Pro achieve the strongest performance, approaching the task-specific MAIRA-2; nevertheless, both still lag substantially behind MedVERSA, which maintains a clear lead across all metrics. 
Notably, GPT-5 and o3—despite substantially outperforming GPT-4o on VQA-style benchmarks—do not exhibit corresponding gains in report generation. This divergence underscores that improvements in general multimodal VQA do not necessarily translate into better radiology report generation, a task that demands precise identification of clinical findings, faithful spatial grounding, and disciplined use of domain-specific terminology.

\clearpage
\vspace{5mm}
\section{Prompt Design}
\label{app:Prompt}

% Prompts used for Sec \ref{sec:stress-tests}
This appendix details the prompt formulations used in Sec \ref{sec:stress-tests}, which were designed to evaluate model performance across different tasks. The report generation prompt follows the structured medical reporting paradigm described in recent work~\cite{jiang-etal-2025-gpt}. 

\vspace{3mm}
\begin{minipage}{0.95\linewidth}
    \begin{dialogbox}[Multiple Choice Prompt]
        \footnotesize
         \textcolor{darkbrown}{\# User prompt}\\
         <Images> \\
         You are a helpful medical assistant that answers multiple choice questions about the provided image. The following is a multiple choice question (with answers). \\
         Question: <Question>\\
         Options: \\
         A. <Option A>\\
         B. <Option B>\\
         ... 

         Please only answer with the index and content of the option. 
    \end{dialogbox}
\end{minipage}


\begin{minipage}{0.95\linewidth}
    \begin{dialogbox}[Multiple Choice Prompt with CoT]
        \footnotesize
         \textcolor{darkbrown}{\# User prompt}\\
         <Images> \\
         You are a helpful medical assistant that answers multiple choice questions about the provided image. The following is a multiple choice question (with answers). \\
         Question: <Question>\\
         Options: \\
         A. <Option A>\\
         B. <Option B>\\
         ... 
         
         Let us think step by step, enclosing the thought process within <thinking> and </thinking>. Provide answer with the index and content of the option, and place it within <answer> and </answer>.
    \end{dialogbox}
\end{minipage}


\begin{minipage}{0.95\linewidth}
    \begin{dialogbox}[Report Generation Prompt]
        \footnotesize
         \textcolor{darkbrown}{\# System prompt}\\
         You are a professional chest radiologist that reads chest X-ray image(s).\\ 
         \\
         \textcolor{darkbrown}{\# User prompt}\\
         <Images> \\
         Below is INDICATION related to chest X-ray images. \\
         INDICATION: \{\} \\
         Write a report that contains only the FINDINGS and IMPRESSION sections based on the attached images and INDICATION. Provide only your generated report, without any additional explanation and special format. Your answer is for reference only and is not used for actual diagnosis.
    \end{dialogbox}
\end{minipage}

==> arxiv2510/sections_v2/benchmark.tex <==
\section*{2. Beyond Leaderboards: Benchmark Evaluation and Behavioral Divergence}
% 
Benchmark leaderboards have become the \textit{de facto} measure of progress in health AI. Yet high scores alone provide an incomplete---and often misleading---picture of model readiness for real-world clinical integration. To understand how performance metrics align with model robustness, we systematically evaluated six leading multimodal models across a representative spectrum of clinical tasks.

We selected benchmarks spanning three core task families:  
(i) \textit{Short-form visual question answering (VQA)}: \textit{VQA-RAD~\cite{lau2018dataset}} , \textit{PMC-VQA}, and \textit{OmniMedVQA};  
(ii) \textit{Long-form report generation}: \textit{MIMIC-CXR};  
(iii) \textit{Complex diagnostic reasoning}: \textit{JAMA} and \textit{NEJM} multiple-choice question sets, designed to reflect real-world clinical problem-solving.

The models evaluated included GPT-4o, GPT-o3, Gemini 2.5 Pro, DeepSeek R1, LLaVaMed 1.5, and ensemble variants. All models were tested under standardized prompting and evaluation conditions to ensure comparability.

Despite similar aggregate accuracy across tasks (Fig.~\ref{fig:benchmark-accuracy}), we observed marked differences in behavior that raise concerns about generalization and reliability. Reasoning-native large multimodal models ---GPT-o3 and Gemini 2.5 Pro---consistently outperformed GPT-4o and all open-source baselines, with a mean absolute accuracy improvement of +11.7 percentage points and +9.4 percentage points, respectively. 

By contrast, DeepSeek R1, which performs competitively on general-domain benchmarks, its accuracy on \textit{JAMA} and \textit{NEJM} was 38.21\% and 33.16\%, respectively—close to random for five-choice questions. This underperformance likely reflects limited biomedical pretraining and modality alignment for medical data. LLaVaMed 1.5, a much smaller vision-language model trained on biomedical corpus and benchmarks, performed moderate on specific tasks (VQA-Rad, OmniMedVQA), but failed to generalize to structurally similar tasks such as \textit{PMC-VQA} (\(6.17\%\) accuracy, failing to produce meaningful answers), indicating strong format overfitting and limited transferability.

Notably, a simple ensemble of GPT-o3 and Gemini 2.5 Pro—using majority voting across model outputs—achieved the highest overall performance across benchmarks (Fig.). However, this performance gain came without interpretability or behavioral improvement: ensembles aggregate outputs but do not mitigate failure modes such as hallucinated reasoning, modality overreliance, or format memorization. While effective in the narrow context of leaderboard optimization, ensemble methods fall short of addressing the core challenges of robustness, transparency, and clinical applicability.

These findings highlight that similar benchmark scores can mask substantial differences in model behavior. Such \textbf{behavioral heterogeneity}—divergent reliance on modality, prompt sensitivity, or domain-specific overfitting—is not captured by current leaderboard reporting. For example, contrary to common assumptions, adding chain-of-thought prompting consistently decreased accuracy on \textit{VQA-RAD} across all models tested (by 6--9 percentage points; Fig.~3b), introducing hallucinated rationales that undermined correct responses. Ensembling, while effective for achieving best leaderboard performance, did not resolve any of these failure modes. Instead, it illustrates a broader limitation of score-based evaluation: \textit{accuracy can rise even as reliability remains opaque}. This motivates a deeper examination of model behavior under stress, addressed in the next section.
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{fig.eps}
    \caption{\textbf{From Leaderboards to Clinical Readiness.} 
Today's evaluation practices in health AI are dominated by aggregate benchmark scores (left), which often conceal brittle or misleading behaviors. Models may succeed by memorizing patterns or ignoring multimodal input. Our proposed framework (right) emphasizes clinically grounded evaluation dimensions—reasoning complexity, visual dependency, and robustness under perturbation—that better align with real-world clinical demands.}
    \label{fig:benchmark-gap}
\end{figure}
\begin{table}[ht]
\centering
\caption{(Extended Table) Model performance across clinical benchmarks. Accuracy is reported as percentages. Highest-performing ensemble is outlined in gold in Fig.~2.}
\label{tab:benchmark_performance}
\begin{tabular}{lcccccc}
\toprule
{} & VQA-RAD &  PMC-VQA &  OmniMedVQA &   JAMA &   NEJM & MIMIC-CXR \\

\midrule
GPT-4o         &   60.98 &    50.21 &       73.31 &  69.94 &  66.90 &      67.0 \\
GPT-o3         &   65.63 &    60.08 &       85.49 &  84.75 &  80.89 &      60.2 \\
GPT-o4-mini    &   64.08 &    59.47 &       81.43 &  80.46 &  75.91 &      62.6 \\
Gemini-2.5-pro &    66.3 &    58.44 &       85.69 &  84.84 &  83.74 &      64.8 \\
DeepSeek       &   45.68 &    40.95 &       54.01 &  38.21 &  33.16 &      49.6 \\
LLaVaMed-1.5   &   44.35 &     6.17 &       68.66 &  22.74 &  29.04 &         - \\
Ensemble       &       - &    62.76 &       87.62 &  86.06 &  81.83 &         - \\
\bottomrule
\end{tabular}
\end{table}


==> arxiv2510/sections_v2/discussion.tex <==
\section{Rethinking Progress: Towards Real-world Readiness}

Across previous sections, we have shown that current benchmarks often overstate model readiness. Despite impressive leaderboard scores, many leading models 
exhibit inconsistent behavior, reliance on superficial patterns, and fragile reasoning under mild input perturbations. These findings challenge the prevailing assumption that benchmark success signals medical viability.

\subsection*{I. The False Signal of Benchmark Scores}

Today's benchmarks offer a convenient but incomplete lens into model capability. Their design often emphasizes answer correctness while ignoring whether the answer is reached through medically valid reasoning, multimodal understanding, or robust generalization. As demonstrated in our stress tests, models can perform well by leveraging shallow cues—such as positional biases in answer options or memorized response formats—without engaging meaningfully with the underlying medical content.

Such behaviors are not easily detected by conventional metrics. For example, reasoning models may improve benchmark scores while still producing hallucinated or implausible rationales. Reinforcement learning approaches may optimize for token-level reward signals rather than faithful reasoning. The result is a misleading sense of progress: \textbf{performance improves numerically, but not behaviorally.}

\subsection*{II. Redefining Readiness in the Medical Context}

Medical readiness is a multidimensional construct. In real-world settings, models must tolerate missing or noisy data, justify their decisions in a manner clinicians can understand, and reason across time, modality, and context. Performance must be not only accurate but also reliable, interpretable, and safe under uncertainty.

Unlike domains such as mathematics or programming, where ground truth is unambiguous and logic is formal, healthcare requires flexible, contextual reasoning. Attempts to port reasoning strategies from other domains—such as multi-agent planning or chain-of-thought prompting—often fall short in medicine, where \textbf{ambiguity, incomplete information, and medical nuance are the norm}. Without alignment to this reality, advances in model capability risk being confined to artificial test settings.

\subsection*{III. Stress Testing as a Foundation for Trustworthy Evaluation}

Static benchmark scores provide little insight into how models behave under real-world uncertainty.  
To address this limitation, we propose \textbf{structured stress testing} as a core component of evaluation.  
As shown in Section~\ref{sec:stress-tests}, our tests T1–T5 revealed distinct vulnerabilities—models often \textbf{succeed for the wrong reasons}, retaining high accuracy even when visual input is removed (T1–T2, see Example ~\ref{fig:no_image_example_1}-\ref{fig:no_image_example_3}); they show \textbf{brittle behavior} under minor perturbations such as distractor reordering, weakening, or visual substitution (T3–T5, See Example ~\ref{fig:no_image_example_1}-\ref{fig:image_replaced_example_3}); and they frequently produce \textbf{fabricated reasoning chains}, generating confident but incorrect explanations that mask underlying shortcut behaviors (T6, See Example ~\ref{fig:error_reason_heuristic}-\ref{fig:error_reason_misgrounded}).    
These fragilities were hidden in leaderboard performance alone.

We generalize this approach into a framework of modular tests, each targeting a specific vulnerability such as neglect of visual input, dependence on spurious answer patterns, or overconfident reasoning when evidence is absent.  
By isolating these behaviors, stress tests enable systematic comparison across models and tasks, offering a principled means of diagnosing brittleness that static benchmarks obscure.  
In doing so, they establish a foundation for evaluation protocols that move beyond leaderboards and toward measures of robustness and trustworthiness.


\subsection*{IV. Toward Community Standards for Evaluation Reform}

We propose several actionable recommendations for the field:

First, benchmarks should be accompanied by metadata that characterizes their reasoning and visual complexity, using structured rubrics like those presented in Section~3. This allows model performance to be interpreted in medically meaningful dimensions rather than aggregated scores alone.

Second, evaluation protocols should routinely incorporate adversarial and stress-based assessments, particularly for models intended for high-stakes deployment. These assessments should be reported alongside accuracy metrics and form the basis of model release audits.

Third, the field must shift its mindset: benchmarks are tools for assess, not endpoints. Their role is to \textbf{reveal model capabilities and limitations under realistic constraints—not to be optimized at the cost of generalization.}

As large multimodal models continue to advance, our ability to test them meaningfully must evolve in parallel. Stress testing offers a path forward, grounded not in artificial difficulty, but in the realities of real world.


==> arxiv2510/sections_v2/extended.tex <==
\clearpage
\section*{Extended Data}
\captionsetup[figure]{labelfont=bf,labelsep=space,name=Extended Data Fig.}
\captionsetup[table]{labelfont=bf,labelsep=space,name=Extended Data Table}

\begin{table}[ht]
\centering
\caption{\textbf{Benchmark leaderboard accuracy, (\%) across representative multimodal medical benchmarks.}}
\label{tab:leaderboard_main}
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{VQA-RAD} & \textbf{PMC-VQA} & \textbf{OmniMedVQA} & \textbf{JAMA} & \textbf{NEJM} \\
\midrule
\textbf{GPT-5}        & \textbf{67.85} & 58.85 & \textbf{87.43} & \textbf{86.59} & \textbf{80.89} \\
Gemini-2.5 Pro        & 66.30 & 58.44 & 85.69 & 84.84 & 79.95 \\
OpenAI-o3                & 65.63 & 60.08 & 85.49 & 84.75 & \textbf{80.89} \\
OpenAI-o4-mini          & 64.08 & 59.47 & 81.43 & 80.46 & 75.91 \\
GPT-4o                & 60.98 & 50.21 & 73.31 & 69.94 & 66.90 \\
DeepSeek-VL2          & 45.68 & 40.95 & 54.01 & 38.21 & 33.16 \\
LLaVA-Med-1.5         & 44.35 & 6.17  & 68.66 & --    & -- \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\caption{\textbf{Stress Test 1: Modality Sensitivity.}
Accuracy (\%) of models on filtered subsets of \textit{JAMA} (1{,}141 items) and \textit{NEJM} (743 items) under \textit{Image+Text} and \textit{Text Only} conditions. $\Delta$ denotes the change in accuracy (\textit{Text Only} $-$ \textit{Image+Text}).}
\label{tab:stress1_modality_sensitivity}
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Model} & \multicolumn{3}{c}{\textbf{JAMA}} & \multicolumn{3}{c}{\textbf{NEJM}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & Img+Txt & Txt Only & $\Delta$ & Img+Txt & Txt Only & $\Delta$ \\
\midrule
\textbf{GPT-5 }         & 86.59 & 82.91 & -3.68  & 80.89 & 67.56 & -13.33 \\
Gemini-2.5 Pro & 84.84 & 74.93 & -9.91  & 79.95 & 65.01 & -14.94 \\
OpenAI-o3         & 84.75 & 82.65 & -2.10  & 80.89 & 67.03 & -13.86 \\
OpenAI-o4-mini   & 80.46 & 78.44 & -2.02  & 75.91 & 66.49 & -9.42  \\
GPT-4o         & 69.94 & 68.89 & -1.05  & 66.90 & 37.28 & -29.62 \\
DeepSeek-VL2   & 38.21 & 32.60 & -5.61  & 33.16    & 25.30 & -7.86     \\
LLaVA-Med-1.5  & 22.74 & --     & --     & --    & --    & --     \\
\bottomrule
\end{tabular}

\vspace{0.5em}
\begin{minipage}{0.95\textwidth}
\footnotesize
\textbf{Notes:} (i) Two-decimal precision preserved from raw logs; $\Delta$ computed as exact subtraction (two decimals). 
(ii) For \textit{NEJM}, \textbf{DeepSeek-VL2} and \textbf{LLaVA-Med-1.5} lacked filtered \textit{Image+Text} results (743); hence cells are “--”. 
If you prefer to include \textit{unfiltered} NEJM entries for completeness: DeepSeek-VL2 \textit{Img+Txt}=33.16 (N=947), yielding $\Delta=-7.86$ with \textit{Txt Only}=25.30; LLaVA-Med-1.5 \textit{Img+Txt}=29.04 (N=947), no \textit{Txt Only} available.
\end{minipage}
\end{table}


\begin{table}[htbp]
\centering
\caption{\textbf{Stress Test 2: Modality Necessity.}  
Accuracy (\%) of models on a manually curated NEJM subset where correct answers require visual input.  
A visually grounded model should perform near the 20\% random baseline in the \textit{Text Only} setting.  
Most models significantly exceed this threshold. GPT-4o performs well below chance due to refusal behavior.}
\label{tab:stress2_modality_necessity}
\small
\begin{tabular}{lrr}
\toprule
\textbf{Model} & \textbf{Image+Text (\%)} & \textbf{Text Only (\%)} \\
\midrule
Chance Level   & --     & 20.0 \\
\midrule
\textbf{GPT-5 }         & 66.3   & \textbf{37.7} \\
Gemini-2.5 Pro & 67.4   & \textbf{37.1} \\
OpenAI-o3         & 61.7   & \textbf{37.7} \\
OpenAI-o4-mini   & 58.9   & \textbf{33.7} \\
GPT-4o         & 46.3   & \textbf{3.4}\textsuperscript{†} \\
\bottomrule
\end{tabular}

\vspace{0.5em}
\begin{minipage}{\linewidth}
\footnotesize
\textbf{Note:} Most models exceed the 20\% random baseline when images are removed, indicating shortcut behavior via learned text-pattern correlations.  
\textsuperscript{†}GPT-4o's score reflects refusal behavior (e.g., declining to select from the answer options when visual input is missing), resulting in accuracy below chance.
\end{minipage}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Stress Test 3: Format Perturbation.}  
Accuracy (\%) on a visually-required NEJM subset before and after random reordering of answer choices.  
Reordering weakens shortcut patterns (e.g., fixed answer positions), reducing accuracy in the \textit{Text} condition.  
In contrast, \textit{Image+Text} performance is stable or slightly improved, suggesting vision becomes more informative when textual cues are disrupted.}

\label{tab:stress3_format_perturbation}
\small
\begin{tabular}{lrrrr}
\toprule
\textbf{Model} 
& \textbf{Text (orig)} 
& \textbf{Text (reord)} 
& \textbf{Img+Txt (orig)} 
& \textbf{Img+Txt (reord)} \\
\midrule
\textbf{GPT-5 }         & 37.71 & \textbf{32.00} & 66.28 & 70.85 \\
Gemini-2.5 Pro & 37.14 & \textbf{33.14} & 67.42 & 70.28 \\
OpenAI-o3         & 37.71 & \textbf{31.42} & 61.71 & 64.00 \\
OpenAI-o4-mini   & 33.71 & 33.71          & 58.86 & 55.43 \\
GPT-4o         & 3.43  & \textbf{0.57}\textsuperscript{†} & 46.29 & 46.85 \\
\bottomrule
\end{tabular}

\vspace{0.5em}
\begin{minipage}{\linewidth}
\footnotesize
\textbf{Note:} Reordering answer options should not affect accuracy.  
Accuracy drops in the \textit{Text Only} condition reveal shortcut reliance on answer format or position.  
\textit{Image+Text} performance improves slightly, indicating vision is used more when textual cues weaken.  
\textsuperscript{†}GPT-4o frequently refused to answer in the perturbed text-only condition.
\end{minipage}
\end{table}

\begin{table}[htbp]
\centering
\caption{\textbf{Stress Test 4: Robustness to Distractor Perturbations.}
Prompt options are modified by replacing 1–4 distractors with plausible alternatives (1R–4R), or one with the string \texttt{"unknown"} (UNK).
All variants preserve the ground truth.
Accuracy is reported for both text-only and multimodal inputs.}
\label{tab:stress4_full}
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Model} & \textbf{Base} & \textbf{UNK} & \textbf{1R} & \textbf{2R} & \textbf{3R} & \textbf{4R} \\
\midrule
\multicolumn{7}{l}{\textit{Text Only}} \\
\midrule
\textbf{GPT-5 }          & 37.71 & 42.86 & 33.14 & 29.24 & 24.27 & 20.00 \\
Gemini-2.5 Pro  & 37.14 & 45.71 & 38.86 & 35.42 & 26.85 & 17.14 \\
OpenAI-o3          & 37.71 & 34.28 & 29.71 & 27.42 & 21.14 & 20.00 \\
OpenAI-o4-mini    & 33.71 & 42.28 & 36.57 & 32.57 & 24.57 & 17.14 \\
GPT-4o          &  3.43 &  4.57 &  1.71 &  2.28 &  0.37 &  2.28 \\
\midrule
\multicolumn{7}{l}{\textit{Image + Text}} \\
\midrule
\textbf{GPT-5 }          & 66.28 & 71.73 & 69.71 & 73.71 & 86.29 & 90.86 \\
Gemini-2.5 Pro  & 67.43 & 69.71 & 72.00 & 73.71 & 82.29 & 92.57 \\
OpenAI-o3          & 61.71 & 67.43 & 68.57 & 70.86 & 80.57 & 89.14 \\
OpenAI-o4-mini    & 58.86 & 61.14 & 62.37 & 68.57 & 73.72 & 85.14 \\
GPT-4o          & 46.29 & 53.71 & 50.28 & 54.28 & 65.14 & 84.00 \\
\bottomrule
\end{tabular}

\vspace{0.5em}
\begin{minipage}{\linewidth}
\footnotesize
\textbf{Interpretation:} In text-only settings, accuracy declines as more incorrect options are replaced (1R–4R), indicating reliance on shallow lexical patterns. Notably, inserting a single \texttt{"unknown"} distractor improves performance, suggesting models may exploit pattern-based elimination heuristics. In contrast, image+text performance improves with increased distractor replacement, implying that visual grounding becomes more influential when shortcut signals are weakened.
\end{minipage}
\end{table}


\begin{table}[ht]
\centering
\caption{\textbf{Stress Test 5: Visual Substitution.} Accuracy on NEJM items when the original image is replaced with one that supports a distractor option, while the question and answer choices remain unchanged. This isolates whether models exhibit genuine visual understanding or rely on memorized visual–answer associations.}
\vspace{0.5em}
\small
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Original (\%)} & \textbf{Image Subst. (\%)} & \textbf{$\Delta$ Acc. (pp)} \\
\midrule
\textbf{GPT-5 }          & 83.33 & 51.67 & \textbf{-31.66} \\
Gemini-2.5 Pro  & 80.83 & 47.50 & \textbf{-33.33} \\
OpenAI-o3          & 76.67 & 52.50 & \textbf{-24.17} \\
o4-mini         & 71.67 & 37.50 & \textbf{-34.17} \\
GPT-4o          & 36.67 & 41.67 & \textbf{+5.00} \\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption*{\footnotesize \textbf{Note:} Models with genuine visual understanding should revise their prediction when the image is changed to support a different answer. Instead, performance drops sharply—especially for top-performing models—suggesting reliance on shortcut visual–answer associations rather than robust image interpretation.}
\label{tab:stress5_visualsubs}
\end{table}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig_rubric_reason.pdf}
        \caption{Reasoning complexity rubric, scored along five sub-axes reflecting depth of inference, uncertainty, and clinical decision impact.}
        \label{fig:rubric_reasoning}
    \end{subfigure}
    \vspace{1em}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig_rubric_visual.pdf}
        \caption{Visual complexity rubric, capturing task reliance on detailed image interpretation, spatial understanding, and visual comparison.}
        \label{fig:rubric_visual}
    \end{subfigure}
    \caption{\textbf{Clinician-defined rubrics for evaluating benchmark complexity.} These rubrics enable systematic profiling of benchmarks along clinically relevant reasoning and visual dimensions, revealing variation that standard metadata overlooks.}
    \label{fig:rubric_combined}
\end{figure}

\begin{table}[ht]
\centering
\caption{\textbf{Performance evaluation on chest X-ray report generation using the MIMIC-CXR dataset.} Best in bold, second-best underlined.}
\vspace{0.5em}
\small
\begin{tabular}{lccccc}
\hline
Model & 1/RadCliQ-v1 & BLEU Score & BERT Score & Semantic Score & RadGraph F1\\
\hline
GPT-4V & 0.558 & 0.068 & 0.207 & 0.214 & 0.084\\
GPT-4o & 0.670 & 0.098 & 0.289 & 0.291 & \underline{0.153}\\
GPT-5 & 0.628 & 0.090  & 0.251 & 0.271 & 0.140 \\
o3 & 0.596 & 0.084 & 0.210 & 0.260 & 0.135 \\
% o3 (high) & 0.602 & 0.085 & 0.217 & 0.264 & 0.136 \\
o4-mini & 0.626 & 0.091 & 0.233 & 0.284 & 0.148 \\
Gemini-2.5-pro & 0.648 & \underline{0.100} & 0.257 & 0.307 & 0.143 \\
Deepseek & 0.496 & 0.047 & 0.094 & 0.198  & 0.066 \\
MAIRA-2 & \underline{0.694} & 0.088 & \underline{0.308} & \underline{0.339} & 0.131\\
MedVERSA & \textbf{1.103} & \textbf{0.209} & \textbf{0.448} & \textbf{0.466} & \textbf{0.273}\\
\hline
\end{tabular}
\vspace{0.5em}
\caption*{\footnotesize \textbf{Note:} We report quantitative results for GPT-4V, MAIRA-2, and MedVERSA based on the ReXrank leaderboard~\cite{zhang2024rexrank}, which provides standardized evaluation for AI-powered chest X-ray radiology report generation.}
\label{tab:report_evaluation}
\end{table}

==> arxiv2510/sections_v2/intro.tex <==
\section{Introduction: The Illusion of Readiness in Health AI}

% Large language models (LLMs) and large multimodal models (LMMs) are poised to reshape healthcare by enabling richer, more flexible interactions with complex medical data. These models can now interpret text, images, and structured inputs at scale, achieving expert-level performance on synthetic exams and medical question-answering tasks. Yet despite their apparent success, real-world deployment remains rare. Models that excel on standard benchmarks frequently underperform in medical settings, where ambiguity, context, and multimodal integration are the norm.

% This gap between benchmark performance and medical readiness is more than an implementation lag—it reflects a deeper misalignment between what benchmarks test and what real-world use demands. Current evaluation practices often center on simplified question-answering tasks, idealized vignettes, or sanitized case formats that fail to capture the nuance and variability of actual patient care. These benchmarks may reward superficial pattern recognition or dataset memorization rather than robust, verifiable reasoning. As a result, they can give a false sense of model reliability and safety.

% Healthcare poses unique evaluation challenges. medical decisions are rarely binary; they often involve incomplete information, competing hypotheses, and evolving temporal dynamics. Visual reasoning—from identifying subtle findings in radiology images to comparing multi-view scans—is critical across specialties, yet remains underrepresented in benchmark design. Similarly, benchmarks rarely assess how models handle uncertainty, explain their rationales, or perform under adversarial or perturbed input—core components of trustworthiness in medical environments.

% In this paper, we argue that the current benchmark paradigm is insufficient. We show that many state-of-the-art models behave unpredictably when evaluated under real-world stressors. These failures are not random: they reveal hidden dependencies on benchmark structure and highlight the mismatch between synthetic test formats and medical cognition.

% To bridge this gap, we contribute a structured analysis across three dimensions:

% \begin{itemize}
%     \item \textbf{Stress-testing model robustness:} We introduce a suite of stress tests that simulate medical constraints, revealing how high-scoring models often rely on spurious cues or fragile heuristics.
%     \item \textbf{Clinician-labeled benchmark profiling:} We annotate widely used benchmarks along key axes of reasoning complexity and visual dependency, uncovering substantial variation that standard metrics overlook.
%     \item \textbf{Toward trustworthy evaluation:} We propose a roadmap for more meaningful benchmarking in health AI, grounded in medical realism, reasoning verifiability, and stress-informed performance diagnostics.
% \end{itemize}

% By revealing the hidden fragilities beneath benchmark success, our goal is to refocus evaluation toward medical robustness—not leaderboard optimization. We advocate for evaluation methods that reflect the complexities of care delivery and the real demands placed on decision-support tools. Only then can we ensure that model progress translates to safer, more reliable health AI.


Health AI has a credibility problem. Models like GPT-5~\cite{openai_gpt5} can ace medical exams and top multimodal benchmarks yet still falter on simpler tasks, such as preserving their answers when answer choices are shuffled, or justifying their predictions with medically sound reasoning. This isn't just an implementation lag. \textbf{We're measuring the wrong things}.

Current health AI benchmarks reward test-taking strategies rather than robust medical cross-modal understanding~\cite{griot-etal-2025-pattern}. A model might diagnose pneumonia not by interpreting radiologic features, but by learning that “productive cough + fever” statistically co-occurs with pneumonia in training data. This is shortcut learning, not medical understanding.
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures_v2/figure1_v3.pdf}
\caption{\textbf{Stress tests reveal hidden fragilities in LMMs on multimodal medical tasks.}  
\textbf{a.} Conceptual illustration: Benchmark scores suggest steady model improvement. Stress tests uncover hidden vulnerabilities—newer models may be equally or more brittle despite higher scores.  
\textbf{b.} While conventional benchmark scores (green line) show progress, robustness scores (red line) expose increasing brittleness under incomplete or adversarial inputs.  
\textbf{c.} Stress test heatmap disrupts the apparent leaderboard, revealing model-specific failure patterns.  
\textbf{d.} Illustrative examples: (1) correct answer despite missing image and shuffled choices (shortcut behavior); (2) fabricated rationale when asked to explain an answer without visual input.}

\vspace{-1em}
\captionsetup{format=plain}
\caption*{\footnotesize\textit{Note: Panel d examples are generated from GPT-5 responses when prompted post hoc for reasoning. Response variability may occur across runs. To enforce direct answering, all prompts included the suffix: “Please only answer with the index and content of the option.” See Appendix~\ref{app:Prompt}: Prompt Design.}}

\label{fig:mainfragilities}
\end{figure}

When we looked deeper, the problems became clear:

\begin{itemize}
    \item \textbf{Models succeed for the wrong reasons:} On multimodal medical benchmarks~\cite{nejm_image_challenge,jama_challenge}, leading models retained most of their original accuracy even when images were removed. For questions that explicitly require visual input, they still guess correctly, with cues as minimal as a single familiar distractor.
    \item \textbf{Brittle performance:} Reordering answer choices, weakening distractors, or subtly changing the image causes large shifts in predictions, despite no change to the core medical question.
    \item \textbf{Fabricated reasoning:} Models trained to “think step by step”~\cite{openai_reasoning_guide} often paired confident rationales with incorrect logic producing medically sound explanations for wrong answers, or correct answers supported by fabricated reasoning.
\end{itemize}

These aren't minor technical glitches. They reveal fundamental problems with how we evaluate and incentivize progress in health AI. Current benchmarks test pattern matching, not medical understanding. They reward consistency on test formats rather than robustness under real medical conditions.

Real-world medical decisions are made under uncertainty, incomplete information, and high stakes. If a model fails when answer choices are shuffled, how can we trust it with ambiguous symptoms or noisy imaging? Benchmarks don’t just evaluate models but shape how they’re trained and optimized~\cite{openai2025hallucinate}. When benchmarks reward test-taking shortcuts over genuine medical understanding, they create misleading signals of progress.

This paper exposes these fragilities through a series of targeted stress tests across six high-profile models and six widely used multimodal medical benchmarks. We show that state-of-the-art scores can hide medical brittleness and that model performance is often benchmark-specific, driven by exploiting artifacts rather than generalizable capability.

We then turn to the benchmarks themselves. 
Through structured clinician-guided analysis, we profile benchmark demands across reasoning complexity and visual dependency. The findings are striking: widely used benchmarks vary widely in what they actually test, yet are treated interchangeably in model evaluation. This masks key failure modes and risks misrepresenting real-world readiness.


Our findings call for a fundamental reevaluation of how we measure progress in health AI. Before these systems are used to support medical decision making, we must ensure they succeed for the right reasons, not merely because they can pass a test.

% To that end, we apply a series of stress tests that strip away spurious cues and shortcut opportunities. Even under these stricter conditions, performance improves steadily across model iterations, indicating that newer models are making genuine capability gains. However, the gains are modest, suggesting that progress may be approaching a bottleneck and that further advances could require new methods or data.
To that end, we apply a series of targeted stress tests that strip away spurious cues and shortcut opportunities. Even under these stricter conditions, performance improves across model generations—indicating real capability gains. But the gains are modest, and the brittleness persists. Further progress will require not just better models, but better ways to evaluate them.




==> arxiv2510/sections_v2/method.tex <==
\section{Methods}

\subsection{Stress–test protocols}
\textbf{Test 1 (Modality ablation, dataset level).} Each item is run twice: \emph{image+text} vs.\ \emph{text–only} (image removed).\\
\textbf{Test 2 (Visual necessity, vision–critical subset).} On \textit{NEJM-175}, models answer with \emph{text–only}; for completeness we also report \emph{image+text} on the same items.\\
\textbf{Test 3 (Answer–option reordering).} For each item, we permute the order of the five options while keeping stem, image, and option texts unchanged (the correct option's text is preserved, only its position changes). We use at least one random permutation per item; where multiple permutations are available, we aggregate across $K$ permutations.\\
\textbf{Test 4 (Distractor replacement).} For each item, we progressively replace $r\in\{0,1,2,3,4\}$ incorrect options with distractors sampled from other items (without altering the correct option text). We evaluate both \emph{image+text} and \emph{text–only} at each $r$.

\subsection{Metric definitions}
We report simple, transparent metrics. Let $A$ denote accuracy in percent and $c{=}20$ the chance level (5–choice). We normalize above–chance accuracy as
\[
\mathrm{nacc}(A) \;=\; \frac{\max(0,\ A-c)}{100-c}\in[0,1].
\]
\textbf{Visual Grounding Gain (VGG).} Dataset–level image benefit in percentage points:
\[
\mathrm{VGG} \;=\; A_{\text{image+text}} \;-\; \max(A_{\text{text-only}},\, c).
\]
\textbf{No–Image Above–Chance (NIAC).} Text–only surplus over chance on vision–critical items:
\[
\mathrm{NIAC} \;=\; A_{\text{text-only}} \;-\; c \quad (\text{pp}).
\]
\textbf{Reorder Stability (RS).} With per–item predictions, stability for item $i$ is
\[
s_i \;=\; \frac{1}{K}\sum_{k=1}^{K}\mathbf{1}\!\left(y_i^{(k)}=y_i^{\text{orig}}\right), \quad
\mathrm{RS} \;=\; \frac{\sum_i s_i\,\mathbf{1}(\text{orig correct})}{\sum_i \mathbf{1}(\text{orig correct})}.
\]
When only aggregate accuracies are available, we report a conservative proxy
\[
\mathrm{RS}_{\text{agg}} \;=\; 1 - \frac{\big|A_{\text{reordered}}-A_{\text{original}}\big|}{100-c}.
\]
\textbf{Distractor Grounding Advantage (DGA).} Mean normalized advantage of \emph{image+text} over \emph{text–only} as distractors are replaced:
\[
\mathrm{DGA} \;=\; \frac{1}{5}\sum_{r=0}^{4}\Big(\mathrm{nacc}\!\big(A^{\text{full}}(r)\big) - \mathrm{nacc}\!\big(A^{\text{text}}(r)\big)\Big)\ \in[0,1].
\]
For readability in the main text we report DGA in percentage points via $80\times\mathrm{DGA}$.

\subsection*{Composite Stress Robustness (CSR)}
We summarize robustness with a single score combining visual grounding, format stability, and distractor robustness. Let
\[
\mathrm{VGS} \;=\; \mathrm{nacc}\!\big(A^{\text{full}}\big)\cdot \frac{\max\!\big(0,\ A^{\text{full}}-\max(A^{\text{text}},c)\big)}{100-c},
\quad
\mathrm{DRS} \;=\; \operatorname{clip}\!\Big(0.5 + 0.5\big(\overline{\mathrm{nacc}}_{\!r}(A^{\text{full}}) - \overline{\mathrm{nacc}}_{\!r}(A^{\text{text}})\big),\,0,\,1\Big).
\]
We then define
\[
\mathrm{CSR}_{\text{NEJM-175}} \;=\; 100 \times \big(\alpha\,\mathrm{VGS} + \beta\,\mathrm{RS}_{\text{agg}} + \gamma\,\mathrm{DRS}\big),
\]
with weights $\alpha{=}0.6$, $\beta{=}0.2$, $\gamma{=}0.2$ fixed \emph{a priori}. CSR is used for Figure~1A only; all claims in Section~2 rely on the per–test metrics above.

\subsection{Evaluation details}
We use the same item splits for all tests on \textit{NEJM-175}. Each model is evaluated with the original multiple–choice stem and options; images are supplied only in \emph{image+text} conditions. Option reordering preserves option texts (position only). Distractor replacements sample from other items without altering the correct option. All evaluations use a fixed random seed per model; when multiple permutations are available, results are averaged over $K$ permutations. 


==> arxiv2510/sections_v2/related.tex <==
\section{Evaluation Landscape}

==> arxiv2510/sections_v2/rubric.tex <==
\section{Benchmarking the Benchmarks: What Are We Really Measuring?}
\label{sec:benchmark-taxonomy}


Despite similar leaderboard scores, Section~\ref{sec:stress-tests} revealed substantial variation in how models respond to medical stressors—ranging from hallucinated justifications to modality overreliance and format-based shortcuts. These divergent behaviors raise a fundamental question:


\begin{quote}
\textit{If models succeed on benchmarks but fail under stress, what do these benchmarks actually measure—and how can we improve them?}
\end{quote}

To answer this, we systematically analyzed six representative benchmarks using structured clinician input to understand what each benchmark actually tests.


\subsection*{I. Motivation: Stress Test Failures Reveal Benchmark Gaps}

The stress tests in Section~\ref{sec:stress-tests} revealed that high benchmark scores do not guarantee robust model behavior. Models that performed well under standard conditions often failed when subjected to small perturbations—such as removing the image, reordering answer options, replacing distractors, or introducing misleading visual inputs.

Critically, these failure modes varied by benchmark. On \textit{NEJM}, removing visual input led to steep performance drops, suggesting strong dependence on image understanding. In contrast, scores on \textit{JAMA} remained stable—indicating that many items could be answered from text alone. 
% Similarly, chain-of-thought prompting improved performance on \textit{NEJM}, but consistently harmed it on \textit{VQA-RAD}, implying differing reasoning demands. 
Similarly, while chain-of-thought prompting provides explicit reasoning scaffolding that benefits distilled models such as o4-mini, its impact on \textit{NEJM} was substantially greater than on \textit{VQA-RAD}, underscoring the heterogeneous reasoning demands across benchmarks.
In Test 5, even subtle visual substitutions caused top models to confidently choose incorrect answers—highlighting shortcut reliance on visual–answer associations in some datasets but not others.

These patterns suggest that the benchmarks themselves differ not just in modality or task type, but in what they implicitly evaluate: visual grounding, inference complexity, pattern recall, or distractor elimination. Yet, such distinctions are rarely documented in benchmark metadata or considered during evaluation.

Without deeper understanding of what each benchmark tests, we risk misinterpreting leaderboard progress as real-world readiness. To address this, we conduct a structured, clinician-guided audit of nine representative benchmarks~\cite{johnson2019mimic, he2020pathvqa, liu2021slake, zhang2023pmcvqa, yue2023mmmu}.

\subsection*{II. Clinician-Informed Benchmark Profiling}

To better understand what each benchmark actually tests, we developed a structured, clinician-guided rubric spanning ten medically meaningful dimensions. These axes capture key demands surfaced by our stress tests—ranging from reasoning complexity and medical context to uncertainty handling, visual detail, and multi-view alignment. The full rubric is shown in Fig~\ref{fig:rubric_combined}.



Each benchmark was independently annotated by three board-certified clinicians per axis, using a 3-point ordinal scale. We report the median score for each benchmark-axis pair, and measure inter-annotator agreement using Fleiss' $\kappa$~\cite{fleiss1971measuring}. Agreement was moderate to strong across axes (range: 0.67–0.90). Highest agreement was observed on binary-seeming attributes such as \textit{Text-only Solvable} ($\kappa$ = 0.90) and \textit{Clinical Context} ($\kappa$ = 0.86); lower agreement appeared on more subjective dimensions such as \textit{Visual Detail Required} ($\kappa$ = 0.67).



\subsection*{III. Visualizing the Benchmark Landscape}

To summarize the profiling results, we projected each benchmark into a two-dimensional space defined by reasoning and visual complexity (Fig~\ref{fig:scoreplot}). This visualization reveals clear structural differences among commonly used datasets:

\begin{itemize}
    \item \textit{NEJM} tasks rank high in both reasoning and visual demands.
    \item \textit{JAMA} requires substantial reasoning but is mostly text-solvable.
    \item \textit{VQA-RAD}, \textit{PMC-VQA}~\cite{zhang2023pmcvqa} and \textit{MIMIC-CXR}~\cite{johnson2019mimic} are visually dependent but low in inference complexity.
    \item \textit{OmniMedVQA} clusters low in both dimensions.
\end{itemize}

This landscape helps to explain the benchmark-specific failures observed in Section~\ref{sec:stress-tests}. For instance, models trained on \textit{VQA-RAD} may excel at image localization but struggle on diagnosis-oriented tasks like \textit{NEJM}, which require cross-modal reasoning and medical inference.

\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{figures/score_plot_new.png}

\caption{\textbf{Benchmarks differ in reasoning and visual complexity.}  
Clinician-labeled profiles show that widely used multimodal benchmarks vary substantially in the reasoning and visual demands they place on models.  
While datasets like \textit{NEJM} require high visual and inferential complexity, others like \textit{OmniMedVQA} cluster low on both axes.  
These structural differences help explain the benchmark-specific fragilities observed in Section~\ref{sec:stress-tests}, and highlight the risk of treating all benchmarks as interchangeable measures of readiness.}
\label{fig:scoreplot}
\end{figure}

\subsection*{IV. Implications for Model Evaluation and Design}

These findings underscore the need to treat benchmarks not as monolithic performance targets, but as diagnostic tools that reveal distinct capabilities. We outline three implications:

\begin{itemize}
    \item \textbf{Benchmarks should be treated as diagnostic instruments, not goals.} Their assumptions, design intent, and likely failure modes should be documented and communicated.
    \item \textbf{Leaderboard scores should be disaggregated by benchmark profile.} Model performance should be reported along medically meaningful axes, not averaged across heterogeneous tasks.
    \item \textbf{Benchmark selection should reflect intended deployment context.} For example, evaluating generalist models solely on text-solvable datasets like \textit{JAMA} risks overestimating readiness for visual diagnostic tasks like \textit{NEJM}.
\end{itemize}

Without these practices, benchmark-driven progress risks reinforcing narrow optimization and masking fragilities. Our clinician-labeled rubric and benchmark landscape (Fig.~4) offer a roadmap for more targeted and medically relevant evaluation.



==> arxiv2510/sections_v2/stress_test.tex <==
\section{Hidden Fragilities: Stress-Testing Models on Multimodal Medical benchmarks
}
\label{sec:stress-tests}

High benchmark score performance may imply robustness, but actually conceals brittleness under distributional shift, missing data, or subtle perturbations.  We designed a suite of stress tests that simulate uncertainty and reveal the behavioral shortcuts models may rely on. Rather than evaluating only correctness, these tests expose how models respond to degraded, incomplete, or adversarial input, conditions that characterize real-world use in healthcare environments. 

We organize these stress tests into progressive levels of challenge, escalating from missing or misleading input modalities, to perturbations in structural format, and finally to qualitative audits of model reasoning.

\subsection*{Modality Robustness}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures_v2/figure2_modality_robustness.pdf}
%     \caption{\textbf{Stress tests reveal overestimated modality robustness.}  
% \textbf{Left (Stress Test 1).} Accuracy drops when images are removed on two diagnostic benchmarks (NEJM and JAMA), revealing hidden differences in modality sensitivity across models. Performance drops sharply on NEJM but minimally on JAMA, suggesting inconsistent visual dependence across benchmarks.  
% \textbf{Right (Stress Test 2).} Accuracy on 175 NEJM items that require visual input. Most models score far above the 20\% chance level even without access to the image, indicating shortcut reliance or memorization. GPT-4o scores below chance due to refusal behavior.}
    \caption{\textbf{Stress tests reveal overestimated modality robustness.}  
\textbf{Left (Stress Test 1).} Accuracy drops when images are removed from two diagnostic benchmarks (NEJM and JAMA), revealing hidden differences in modality sensitivity across models. Sharp drops on NEJM—but minimal impact on JAMA—suggest inconsistent visual dependence across benchmarks and question types. Light segments show text-only accuracy; dark segments mark the drop from Image+Text. 
\textbf{Right (Stress Test 2).} Performance on 175 NEJM items requiring visual input. Most models exceed the 20\% random baseline even without images, indicating reliance on shortcut cues such as priors, co-occurrence patterns, or memorized QA pairs. GPT-4o performs below chance due to refusal behavior.}
 

    \label{fig:modality}
\end{figure}

\begin{tcolorbox}[stressheader]
\textbf{Stress Test 1: Multimodal sensitivity}
\end{tcolorbox}

\textbf{Objective:} Assess how models respond to removal of image input on multimodal medical benchmarks.

\textbf{Setup:} We evaluate six models (GPT-5, Gemini 2.5 Pro~\cite{comanici2025gemini}, OpenAI-o3~\cite{openai_o3_o4mini}, OpenAI-4o-mini~\cite{openai_o3_o4mini}, GPT-4o~\cite{openai2024gpt4o}, and DeepSeek-VL2~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}) on the NEJM~\cite{nejm_image_challenge} and JAMA~\cite{jama_challenge} benchmarks in two settings: \emph{image+text} (default) and \emph{text-only} (image removed). All benchmarks are multiple-choice questions pairing a brief clinical vignette with one or more medical images (radiology, dermatology, pathology etc). (All test items passed content safety filters.\footnote{Filtered subsets exclude items that triggered moderation due to graphic clinical content.})

\textbf{Results:} Removing images reveals strikingly different behavior across models that otherwise achieve similar benchmark scores.  
On \textbf{NEJM}, GPT-5 scored 80.89 with images and 67.56 without, a 13.33 pp drop.  
Similarly, Gemini 2.5 Pro dropped 14.94 pp (79.95 → 65.01), OpenAI-o3 fell by 13.86 (80.89 → 67.03), GPT-4o showed the largest drop (66.90 → 37.28, -29.62), and OpenAI-o4-mini showed a moderate drop (75.91 → 66.49, -9.42).  
DeepSeek-VL2 performed poorly in both modes (33.16 → 25.30).

On \textbf{JAMA}, absolute scores were higher and changes smaller: GPT-5 dropped 3.68 pp (86.59 → 82.91), Gemini 2.5 Pro dropped the most (84.84 → 74.93, -9.91), OpenAI-o3 dropped 2.10 (84.75 → 82.65), OpenAI-o4-mini dropped 2.10 (80.50 → 78.40), and GPT-4o dropped just 1.00 pp (69.90 → 68.90).  
The smallest deltas were seen in GPT-4o, suggesting either robustness to missing input or limited reliance on visual cues.  
Notably, DeepSeek-VL2 again underperformed (38.20 → 32.60). See Fig ~\ref{fig:modality} and Extended Data Table~\ref{tab:stress1_modality_sensitivity} for details.

\textbf{Interpretation:} This test highlights two key issues. First, models with similar full-input scores diverge sharply when the image is removed, exposing \textbf{hidden differences in modality sensitivity not reflected in benchmark leaderboards}. Second, the benchmarks themselves vary in visual dependence: NEJM scores drop sharply without images, while JAMA scores remain relatively stable indicating that many items may be \textbf{solvable from text alone}. These \textbf{benchmark-level inconsistencies} motivate our item-level modality profiling in Section~\ref{sec:benchmark-taxonomy}.
To better understand whether score drops reflect robustness to missing input or reveal shortcut-based behavior, we next turn to questions where visual input is explicitly required.


\vspace{0.5em}

\begin{tcolorbox}[stressheader]
\textbf{Stress Test 2: Modality necessity}
\end{tcolorbox}

\textbf{Objective:} Test whether models can answer questions that \emph{require both text and image} even when the image is missing, or whether their benchmark success reflects true multimodal ability.

\textbf{Setup:} We curated a 175-item subset from the NEJM benchmark, manually selecting multiple-choice questions that clinicians agreed \textbf{require visual input} to answer. We ensured that the selected items contained no textual cues, so the correct answer required both text and image. We then evaluated model performance under two conditions: \emph{text-only} (image removed) and \emph{image+text}. Models include GPT-5, Gemini-2.5 Pro, OpenAI-o3, OpenAI-4o-mini, GPT-4o, and DeepSeek-VL2. To ensure validity, we filtered out examples with content moderation triggers or ambiguous visual requirements.

\textbf{Results:} All models achieved high scores on \emph{image+text} (e.g., GPT-5: 66.28\%, Gemini-2.5 Pro: 67.42\%, OpenAI-o3: 61.71\%), confirming these items are solvable with full input. However, without the image, models still performed well above random chance (20\%), despite the image being necessary. For example, GPT-5: 37.71\%, OpenAI-4o-mini: 33.71\%, Gemini-2.5 Pro: 37.14\%, OpenAI-o3: 37.71\%, suggesting models exploit non-visual cues or learn shortcut patterns from training data. GPT-4o, in contrast, scored just 3.4\%\ due to frequent refusal to answer when the image was removed. While this deflates its accuracy, it may reflect more cautious behavior when critical visual input is missing, as opposed to relying on spurious textual cues.
See Extended Data Table~\ref{tab:stress2_modality_necessity} for details. 

\textbf{Interpretation:}   This test isolates potential shortcut behavior by focusing only on \emph{visually required} questions—cases where the text alone offers minimal diagnostic context (e.g., \textit{“What is the diagnosis?”}). Yet models still perform well above chance without images, suggesting reliance on dataset artifacts—such as frequency priors, co-occurrence patterns, or memorized question–answer pairs—rather than genuine multimodal medical understanding.
Unlike others, GPT-4o scored far below chance due to frequent abstention, which though penalized numerically, may better reflect appropriate uncertainty when essential visual context is missing (See Fig ~\ref{fig:no_image_example_1} ~\ref{fig:no_image_example_2} ~\ref{fig:no_image_example_3}).

Importantly, this behavior does not imply model malpractice; many benchmark examples are publicly available online, making them susceptible to unintentional memorization during pretraining. More broadly, \textbf{high benchmark performance may not reflect true multimodal understanding but instead arise from spurious cues or memorized associations, overstating model readiness for real-world medical use.}


% revealing that \textbf{performance may not reflect true multimodal understanding but instead shortcut exploitation from textual patterns}. This also exposes a serious failure mode in current benchmarks: models may appear multimodal-capable while ignoring modality-essential inputs. We next probe these shortcut patterns further through targeted input perturbations.




% \vspace{0.5em}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.99\linewidth]
% {figures/figures_new/NEJM_stress_reorder_175_text_visual.png}
% % {figures/NEJM_question_modification_175.png}
% \caption{\emph{Perturbation sensitivity reveals visual grounding in diagnostic reasoning.}
% Accuracy trends on 175 NEJM-style multiple-choice questions requiring visual interpretation. The x-axis denotes increasing answer perturbation—none (original), distractor reordering, and replacement of 1 to 4 incorrect options with random choices. Accuracy is plotted for two input settings: text-only (dashed lines) and text+image (solid lines). Under text-only input, accuracy drops sharply with perturbation, approaching chance levels (20\%), indicating shortcut reliance and memorization. In contrast, access to visual input stabilizes accuracy across perturbations, revealing effective visual grounding in models like OpenAI-o3 and Gemini 2.5 Pro. The divergence highlights benchmark brittleness and the value of multimodal stress testing in exposing model reliance on superficial patterns.}
% \label{fig:pertubation}
% \end{figure}


\vspace{1em}


\subsection*{Shortcut Pattern Disruption}

Stress Tests 1–2 revealed that LMMs often fall back on shortcuts when a modality is missing. We now examine the \textbf{structure of these shortcuts} more directly, introducing targeted input perturbations to break and analyze the superficial patterns underlying model predictions.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures_v2/figure3_perturbation.pdf}
% \caption{\textbf{Stress tests uncover shortcut reliance under perturbation.}  
% \textbf{Left (Stress Test 3).} Accuracy under option reordering drops in the text-only setting (solid lines), but remains stable or improves with image+text input (dashed), suggesting models turn to visual cues only when superficial text patterns are weakened.  
% \textbf{Middle (Stress Test 4).} Accuracy progressively declines as more distractor options are replaced with random alternatives. Performance nears chance only when all distractors are replaced. Replacing a single distractor with an unknown (UNK) token paradoxically boosts performance, encouraging models to guess correctly.  
% \textbf{Right (Stress Test 5).} Accuracy collapses when images are swapped to align with distractor answers. All models except GPT-4o drop by over 30 percentage points, revealing a strong reliance on visual-answer memorization rather than genuine visual understanding.  
% Line styles denote input modality: solid (text-only), dashed (image+text).}
\caption{\textbf{Stress tests uncover shortcut reliance under perturbation.}  
\textbf{Left (Stress Test 3).} Option reordering causes accuracy to drop in the text-only setting (solid lines), exposing sensitivity to answer formatting. In contrast, accuracy is stable or improves under image+text input (dashed), suggesting vision helps override shallow textual heuristics.  
\textbf{Middle (Stress Test 4).} Accuracy declines as more distractors are replaced with irrelevant alternatives. All models approach random guessing when all distractors are substituted. Surprisingly, replacing a single distractor with an “Unknown” option boosts accuracy (+5–8pp), indicating models treat it as a weakened distractor—not an abstention signal.  
\textbf{Right (Stress Test 5).} Accuracy collapses when images are swapped to align with a distractor answer. Despite no textual changes, models fail to revise predictions—dropping over 30pp—highlighting brittle reliance on visual–label pairings rather than robust visual–textual reasoning.  
Line styles denote input modality: solid (text-only), dashed (image+text).}


    \label{fig:perturbation}
\end{figure}
\vspace{0.5em}
\begin{tcolorbox}[stressheader]
\textbf{Stress Test 3: Format Perturbation}
\end{tcolorbox}

\textbf{Objective:} Evaluate whether models rely on answer presentation, such as \textbf{fixed positions or option order}, instead of question content when choosing answers.

\textbf{Setup:} We use the 175 manually curated NEJM items from Stress Test 2, where both text and image are required to answer correctly. The ground truth distribution is approximately uniform, minimizing class imbalance. We modify the multiple-choice options by randomly reordering them (without altering their meaning), to detect position-based bias. The correct answer remains unchanged in each case. We exclude DeepSeek-VL2 due to consistently meaningless outputs. Accuracy is measured under both \emph{text-only} and \emph{image+text} settings.

\textbf{Results:}  
Reordering distractors causes accuracy drops across all models in the \emph{text-only} setting, suggesting reliance on surface-level patterns. For example, GPT-5 falls from 37.71\% to 32.00\%, Gemini 2.5 Pro from 37.14\% to 33.14\%, and OpenAI-o3 from 37.71\% to 31.42\%. In contrast, in the \emph{image+text} setting, most models see a slight accuracy increase (e.g., GPT-5 from 66.28\% to 70.85\%), likely due to stochasticity or reduced distractor interference when vision is available. See Extended Data Table~\ref{tab:stress3_format_perturbation} for details. 

\textbf{Interpretation:}  
This test reveals that models may rely on superficial answer formatting—particularly distractor position—when images are unavailable. In the \emph{text-only} setting, shuffling the option order leads to consistent performance drops (e.g., GPT-5: \(-5.7\) pp, Gemini 2.5 Pro: \(-4.0\) pp, OpenAI-o3: \(-6.3\) pp), suggesting shortcut behavior based on learned answer position patterns or co-occurrence biases, rather than medical understanding.

The ground truth label distribution is approximately uniform, and no answer content was altered—only distractor positions were randomized—ruling out class imbalance as an explanation. These results imply that models may have internalized fixed-format response from pretraining or prior benchmarks.

In the \emph{text+image} setting, performance across most models remains stable or improves slightly. The three most recent models—GPT-5, OpenAI-o3, and Gemini 2.5 Pro—show modest gains (+2 to +4.6 pp), with GPT-5 improving the most. In contrast, GPT-4o and o4-mini remain largely unchanged. While these shifts are relatively small and may reflect stochastic variation, they suggest that visual inputs provide a more stable signal that helps mitigate brittle text-only heuristics. However, this does not imply that vision reliably overrides faulty reasoning—only that performance is less disrupted when additional modality cues are available.

% This test reveals that models often rely on superficial answer patterns such as fixed option positions or template memorization rather than understanding the question. Performance drops in the text-only setting after option shuffling (e.g., GPT-5: -5.7 pp) suggest \textbf{shortcut behavior based on answer format or position}. In contrast, accuracy in the \emph{image+text} setting remains stable or improves slightly, implying that models shift to relying more on visual cues when available. This contrast suggests that visual input can help override faulty text-only heuristics, but also masks underlying fragilities when those heuristics are disrupted.




\vspace{0.3em}
\begin{tcolorbox}[stressheader]
\textbf{Stress Test 4: Distractor Replacement}
\end{tcolorbox}

\textbf{Objective:}  
Test whether models rely on memorized question–option patterns, rather than genuine understanding, to identify answers.

\textbf{Setup:}  
We progressively replace 1–4 distractor options with irrelevant choices sampled from other items from the same dataset. The correct answer remains valid, but its label (e.g., “B”) may shift due to shuffling. We evaluate under both \emph{text-only} and \emph{image+text} conditions. We also include a variant where a single distractor is replaced with the token “Unknown”, effectively weakening the distractor. We reuse the 175 NEJM items from Stress Test 2. 

\textbf{Results:}  
Under \emph{text-only} input, model accuracy declines as more distractors are replaced with irrelevant options, approaching random guessing when all four are replaced. For example, GPT-5 accuracy drops from 37.7\% (no replacement) to 20\% (4 distractors replaced).
Under \emph{image+text} input, the trend is reversed: accuracy increases as more distractors are replaced. GPT-5 improves from 66.3\% to 90.9\% when all distractors are irrelevant.

A variant with a single distractor replaced by “Unknown” also improves performance slightly across models. For instance, GPT-5 improves by +5.25 percentage points. See Extended Data Table~\ref{tab:stress4_full} for details. 

\textbf{Interpretation:}  
This test examines how models behave when familiar distractors are weakened or removed. In the \emph{text-only} setting, replacing distractors with irrelevant options leads to a consistent accuracy drop across all models. As more distractors are substituted, model confidence in correct guesses deteriorates toward chance—e.g., GPT-5 drops from 37.7\% to 20.0\% when all four distractors are replaced. This suggests that models rely heavily on learned question–option associations, frequency priors, or superficial patterns to make educated guesses in the absence of visual cues. While not unreasonable given minimal textual context (e.g., “What is the diagnosis?”), this behavior reveals a brittle dependency on dataset artifacts rather than genuine understanding.

Interestingly, replacing just one distractor with “Unknown” yields a consistent performance boost across all models (e.g., +5 to +8 percentage points), suggesting “Unknown” is not treated as a legitimate answer under incomplete input, but rather as a weakened distractor—effectively making the task easier by reducing ambiguity. Instead of abstaining or flagging uncertainty, frontier models become more confident in selecting the correct answer, further highlighting their elimination-based reasoning strategy.

In the \emph{image+text} condition (full input), performance increases as distractors are replaced—e.g., GPT-5 rises from 66.3\% to 90.9\%, likely reflecting task simplification, as the substituted distractors are not visually aligned or grounded, and thus easier to rule out. Vision appears to become more helpful when spurious textual cues are disrupted.

Collectively, these observations suggest that \textbf{apparent multimodal medical competence may arise from shallow elimination heuristics}, with small perturbations exposing fundamental fragilities in model behavior.

% Taken together, these findings reveal that \textbf{high benchmark accuracy may reflect shortcut-driven elimination heuristics, not robust multimodal understanding, and that even subtle perturbations can drastically alter model behavior and task difficulty.}


% The sharp accuracy drop in the \emph{text-only} condition reveals that models often depend on \textbf{memorized distractor patterns} rather than contextual understanding. When these familiar options are replaced, model confidence collapses toward chance, exposing a brittle reliance on surface cues.

% In contrast, in the \emph{image+text} condition, performance improves as distractors are removed,demonstrating that \textbf{vision is used as a fallback only when textual shortcuts are disrupted}. Once superficial textual cues become ineffective, visual information is more likely to guide the model's prediction. Even replacing a single distractor with ``Unknown'' weakens elimination heuristics enough to boost visual engagement.

% These findings show that models prioritize \textbf{shortcut-driven elimination strategies} over robust multimodal understanding. Vision becomes informative only when spurious textual cues are disrupted.




\vspace{0.5em}
\begin{tcolorbox}[stressheader]
\textbf{Stress Test 5: Visual Substitution}
\end{tcolorbox}

\textbf{Objective:}  
% Isolate and measure whether models rely on visual–answer matching heuristics rather than genuine cross-modal understanding.
Evaluate whether models truly integrate visual and textual information, or instead rely on shallow visual–answer associations learned during training.

\textbf{Setup:}  
% We replace each image with one that visually aligns with a distractor option, while keeping the text and answer choices unchanged.  
% If a model performs proper visual–textual understanding, it should now switch its answer accordingly. Accuracy is measured in this altered \emph{image+text} condition and compared against the original. We manually curated a subset of NEJM items (40 unique questions) for this test, each verified by clinicians.
We manually curated 40 NEJM examples where the correct answer is tightly linked to specific visual features.  
For each item, we substitute the original image with one that aligns with a distractor choice, while keeping the question and answer options unchanged.  
This creates a new “counterfactual” version where the distractor becomes the intended correct answer.  
A model with genuine visual–textual understanding should revise its prediction in response to the changed image.  
We measure performance under this perturbed \emph{image+text} setting and compare against the original.

\textbf{Results:}  
% Most models suffer substantial performance drops when the image is replaced with one aligned to a previous distractor. In this altered setting, the distractor becomes the new ground truth answer, but despite the question and answer choices remaining unchanged, models often fail to revise their predictions accordingly. This reveals poor visual–textual grounding and limited robustness to changes in visual evidence.
Model performance drops sharply in this altered setting—despite the minimal input change.  
For example:
GPT-5 drops from 83.3\% to 51.7\% ($\Delta$ -31.6 pp), and  
Gemini-2.5 Pro falls from 80.8\% to 47.5\% ($\Delta$ -33.3 pp).  
OpenAI-o3 and o4-mini show similar declines (e.g., o4-mini: -34.2 pp).
GPT-4o is an exception, showing minimal change.  

% This indicates a strong reliance on learned visual–answer pairings rather than genuine visual interpretation. See Extended Data Table~\ref{tab:stress5_visualsubs} for details, with illustrative test cases provided in Appendix~\ref{app:stress test}.
These sharp declines suggest that many models rely on learned visual–answer pairings rather than interpreting visual evidence in context.
 See Extended Data Table~\ref{tab:stress5_visualsubs} for details, with illustrative test cases provided in Appendix~\ref{app:stress test}.

\textbf{Interpretation:}  
% This test isolates visual understanding by altering only the image to match a different answer.  
% A model with true image understanding should update its prediction accordingly.  
% However, performance collapses, revealing that models rely on \textbf{visual–answer memorization shortcuts} rather than cross-modal understanding.  
% Benchmark success thus reflects shortcut exploitation—not robust clinical understanding—and may fail under even slight visual shifts.
This test introduces a targeted perturbation designed to minimally alter the question while shifting the intended answer via the image.  
The substantial performance drop across models highlights a brittle reliance on visual–label associations—rather than robust visual–textual integration.

We acknowledge that this perturbation may also change task difficulty, as the new images vary in visual salience or diagnostic ambiguity.  

Nonetheless, the consistent accuracy collapse—despite no change in textual input—suggests that current benchmarks may reward shortcut behavior over genuine visual reasoning.
\textbf{The fact that performance collapses despite unchanged text reveals that high benchmark scores may reflect brittle visual–answer shortcuts, rather than reliable visual reasoning or robust multimodal understanding.}



\subsection*{Reasoning Signal Integrity}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures_v2/fig4.pdf}
    \caption{\textbf{Illustrative reasoning failure modes.} We show three representative patterns identified through manual audit: (1) \textit{Confident but false heuristic}: the model applies a plausible but incorrect prior (e.g., inferring diagnosis from common associations), leading to systematic errors; (2) \textit{Correct answer but hallucinated perception}: the model selects the right answer despite having no access to the image, suggesting shortcut-based behavior; (3) \textit{Thinking with image but misgrounded}: the model engages in step-by-step visual reasoning, but grounds its logic on incorrect or hallucinated features, ultimately producing a confident yet incorrect conclusion.}
    \label{fig:reasoning}
\end{figure}


\vspace{0.5em}

\begin{tcolorbox}[stressheader]
\textbf{Stress Test 6: Reasoning Signal}
\end{tcolorbox}

\textbf{Objective:}  
Characterize the reasoning behavior of multimodal models on multimodal medical benchmarks.

\textbf{Setup:}  
We analyze models from two perspectives. First, we apply Chain-of-Thought (CoT)~\cite{wei2022chain} prompting to around 100 samples from NEJM and VQA-RAD~\cite{lau2018dataset} to test whether explicitly requesting step-by-step reasoning enhances performance. Second, we manually audit model-generated explanations across tasks, examining their factuality, visual grounding, and alignment with final answers. 
We also vary reasoning strength (from low to high) on OmniMedVQA~\cite{hu2024omnimedvqa} using OpenAI-o3 to assess its impact on reasoning quality.

\textbf{Results:}  
Prompting for CoT yields mixed or negative gains. 
% On VQA-RAD, CoT consistently reduces accuracy across models. On NEJM, only modest gains are observed for Gemini, o3, and o4-mini (+1–3 pp), while GPT-5 slightly declines. Similarly, increasing reasoning strength on OmniMedVQA offers only minor improvements without consistent benefit.
On VQA-RAD and NEJM, CoT consistently reduces accuracy across models, except o4-mini (+2–5 pp), likely because its smaller capacity benefits from the explicit reasoning scaffolding that CoT provides. Similarly, increasing reasoning strength on OmniMedVQA offers only minor improvements without consistent benefit.

Manual audits reveal key reasoning failure patterns:
\textbf{Correct answers, incorrect logic}: Models often produce plausible-sounding but factually wrong justifications—e.g., describing nonexistent features in the image or hallucinating visual findings.
\textbf{Reinforced visual misunderstanding}: When initial visual interpretation is flawed, reasoning often amplifies the error rather than correcting it.
\textbf{Interpretable but uninformative steps}: Some models generate structured reasoning steps (e.g., describing regions of the image), but these do not consistently guide the model to the correct answer. See Fig~\ref{fig:reasoning} for illustrative examples and Appendix~\ref{app:reasoning} for additional, distinct cases.

\textbf{Interpretation:}  
Model-generated reasoning in medical benchmarks is often disconnected from true multimodal understanding.  
\textbf{Correct predictions may result from pattern matching rather than reasoning, while rationales may confidently justify hallucinated or incorrect content.}  
Even when visual reasoning appears structured, it frequently lacks functional linkage to the final answer.  
These findings underscore the unreliability of current reasoning signals and motivate a deeper examination of benchmark reasoning demands, which we present in Section~\ref{sec:benchmark-taxonomy}.

\subsection*{Robustness Score}  
For each stress test (T1–T5), we computed a normalized robustness score in the range [0,1], with higher values indicating greater stability under perturbation.  
The mean robustness score was obtained by averaging across the five tests, providing a single measure of how reliably each model withstands missing modalities, format changes, distractor manipulations, and visual substitutions (Fig.~\ref{fig:mainfragilities}).  
Full computational details are provided in Appendix~\ref{app:robustness}.




